Understanding Contrastive Representation Learning through Alignment and Uniformity on the Hypersphere

Contrastive representation learning has been outstandingly successful in practice. In this work, we identify two key properties related to the contrastive loss: (1) alignment (closeness) of features from positive pairs, and (2) uniformity of the induced distribution of the (normalized) features on the hypersphere. We prove that, asymptotically, the contrastive loss optimizes these properties, and analyze their positive effects on downstream tasks. Empirically, we introduce an optimizable metric to quantify each property. Extensive experiments on standard vision and language datasets confirm the strong agreement between both metrics and downstream task performance. Remarkably, directly optimizing for these two metrics leads to representations with comparable or better performance at downstream tasks than contrastive learning. Project Page: https://tongzhouwang.info/hypersphere Code: https://github.com/SsnL/align_uniform , https://github.com/SsnL/moco_align_uniform

==> misc/hypersphere/figuretext/distribution/gaussian_vis.tex <==
%auto-ignore
%!TEX root = ../../main.tex


\begin{figure*}[ht!]\vspace{-1pt}
    \centering
    \hspace{-0.005\linewidth}\includegraphics[width=1.01\linewidth]{figures/gaussian_vis}%
    \vspace{-9pt}
    \caption{Average pairwise $G_{2}$ potential as a measure of uniformity. Each plot shows $10000$ points distributed on $\sphere^1$, obtained via either applying an encoder on \cifar validation set (same as those in Figure~\ref{fig:toy2d}) or sampling from a distribution on $\sphere^1$, as described in plot titles. We show the points with Gaussian KDE and the angles with vMF KDE.} \label{fig:gaussian_vis}\vspace{-6pt}
\end{figure*}


==> misc/hypersphere/figuretext/distribution/toy2d.tex <==
%auto-ignore
%!TEX root = ../../main.tex


\begin{figure*}[t!]\vspace{-1pt}
    \centering
    \begin{subfigure}[b]{\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim=5 5 10 0, clip]{figures/cifar10_init.pdf}%
        \vspace{-5pt}
        \caption{\textbf{Random Initialization.} Linear classification validation accuracy: $12.71\%$.}
    \end{subfigure}
    \begin{subfigure}[b]{\linewidth}
        \centering
        \vspace{1pt}
        \includegraphics[width=\linewidth, trim=5 5 10 0, clip]{figures/cifar10_supervised.pdf}%
        \vspace{-5pt}
        \caption{\textbf{Supervised Predictive Learning.} Linear classification validation accuracy: $57.19\%$. }
    \end{subfigure}
    \begin{subfigure}[b]{\linewidth}
        \centering
        \vspace{1pt}
        \includegraphics[width=\linewidth, trim=5 5 10 0, clip]{figures/cifar10_contrastive_instance_positive.pdf}%
        \vspace{-5pt}
        \caption{\textbf{Unsupervised Contrastive Learning.} Linear classification validation accuracy: $28.60\%$.}
    \end{subfigure}\vspace{-5pt}
    \caption{Representations of \cifar validation set on $\sphere^{1}$.
    \textbf{Alignment analysis: }We show distribution of distance between features of positive pairs (two random augmentations).  \textbf{Uniformity analysis: }We plot feature distributions with Gaussian kernel density estimation (KDE) in $\R^2$ and von~Mises-Fisher (vMF) KDE on angles (\ie, $\arctantwo(y, x)$ for each point $(x, y) \in \sphere^1$). \textbf{Four rightmost plots} visualize feature distributions of selected specific classes. Representation from contrastive learning is both \emph{aligned} (having low positive pair feature distances) and \emph{uniform} (evenly distributed on $\sphere^1$).
    } \label{fig:toy2d}\vspace{-3pt}
\end{figure*}


==> misc/hypersphere/figuretext/experiments/finetune.tex <==
%auto-ignore
%!TEX root = ../../main.tex

\begin{figure*}[t]\vspace{-4pt}
    \centering
    \begin{subfigure}[b]{0.325\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/expr/stl10_finetune_align.pdf}
    \end{subfigure}\hfill%
    \begin{subfigure}[b]{0.325\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/expr/stl10_finetune_unif.pdf}
    \end{subfigure}\hfill%
    \begin{subfigure}[b]{0.325\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/expr/stl10_finetune_both.pdf}
    \end{subfigure}\vspace{-11pt}
    \caption{Finetuning trajectories from an encoder trained with $\lcontr$ using a suboptimal temperature $\tau = 2.5$. Finetuning objectives are weighted combinations of $\lalign(\alpha\narroweq2)$ and $\lunif(t\narroweq2)$. For each intermediate checkpoint, we measure $\lalign$ and $\lunif$ metrics, as well as validation accuracy of a linear classifier trained from scratch on the encoder outputs. $\lunif$ is exponentiated for plotting purpose. \textbf{Left and middle: }Performance degrades if only one of alignment and uniformity is optimized. \textbf{Right: }Accuracy improves when both are optimized.} \label{fig:expr_finetune}\vspace{-7pt}
\end{figure*}

==> misc/hypersphere/figuretext/experiments/lgda_trend.tex <==
%auto-ignore
%!TEX root = ../../main.tex

\begin{figure}[ht]\vspace{-4pt}
    \centering
    \includegraphics[width=0.92\linewidth]{figures/expr/stl10_lgda_trend.pdf}
    \vspace{-12pt}
    \caption{Effect of optimizing different weighted combinations of $\lalign(\alpha\narroweq2)$ and $\lunif(t\narroweq2)$. For each trained encoder, we show the $\lalign$ and $\lunif$ metrics, and validation accuracy of a linear classifier trained on the encoder outputs. $\lunif$ is exponentiated for plotting purposes. } \label{fig:expr_lgda_trend}\vspace{-2pt}
\end{figure}

==> misc/hypersphere/figuretext/experiments/scatter.tex <==
%auto-ignore
%!TEX root = ../../main.tex

\begin{figure*}[t]\vspace{-1pt}
    \centering
    \begin{subfigure}[t]{0.66\linewidth}
        \includegraphics[width=0.49\linewidth, trim=5 5 5 5, clip]{figures/expr/stl10_scatter_linear_output}
        \hfill
        \includegraphics[width=0.49\linewidth, trim=5 5 5 5, clip]{figures/expr/stl10_scatter_5nn_fc7}%
        \vspace{-4pt}
        \caption{$260$ \stl encoders are evaluated with linear classification on output features and $5$-nearest neighbor on \textrm{fc7} activations. Higher accuracy (blue color) is better.}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[t]{0.3265\linewidth}
        \includegraphics[width=\linewidth, trim=5 5 5 5, clip]{figures/expr/nyu_depth_scatter_depth_conv5}%
        \vspace{-4pt}
        \caption{$64$ \nyudepth encoders are evaluated with CNN depth regressors on \textrm{conv5} activations. Lower MSE (blue color) is better.}
    \end{subfigure}\vspace{-7pt}
    \caption{Metrics and performance of all experiments. Each point represents a trained encoder, with its $x$- and $y$-coordinates showing $\lalign$ and $\lunif$ metrics and color showing the performance on validation set. \textbf{Blue} is better for both tasks. Encoders with low $\lalign$ and $\lunif$ are consistently the better performing ones (lower left corners).}\label{fig:expr_scatter}
\end{figure*}

==> misc/hypersphere/figuretext/experiments/tbl_nyudepth.tex <==
%auto-ignore
%!TEX root = ../../main.tex

\vspace{-2pt}%
\newcommand{\factor}{0.95}
\resizebox{
  \ifdim\factor\width>\textwidth
    \textwidth
  \else
    \factor\width
  \fi
}{!}{%
\small
\centering
\newcommand{\mround}[1]{\round{#1}{4}}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{|c||c||c|c|}
    \hline
    & Loss Formula
    & \textrm{conv5} MSE $\downarrow$
    & \textrm{conv4} MSE $\downarrow$
    \\
    \hline\hline

    Best $\lcontr$ only
    & $\lcontr(\tau\narroweq0.1)$
    & \mround{0.7152826189994812}  % \textrm{conv5} :
    & \textbf{\mround{0.7473379969596863}} % \textrm{conv4} $\lcontr(\tau=0.07)$:
    \\
    \hline

    Best $\lalign$ and $\lunif$ only
    & $1.5 \cdot \lalign(\alpha\narroweq2) + 0.5 \cdot \lunif(t\narroweq2)$
    & \textbf{\mround{0.7070135474205017}} % \textrm{conv5} $0.5 \lunif(t\narroweq2) + 1.5 \lalign(\alpha\narroweq2)$:
    & \mround{0.7528420686721802}  % \textrm{conv4} $0.5 \lunif(t=2) + 1.5 \lalign(\alpha=2)$:
    \\
    \hline

    Best among all encoders
    & $1.5 \cdot \lalign(\alpha\narroweq2) + 0.5 \cdot \lunif(t\narroweq2)$
    & \textbf{\mround{0.7070135474205017}} % \textrm{conv5} $0.5 \lunif(t\narroweq2) + 1.5 \lalign(\alpha\narroweq2)$:
    & \mround{0.7528420686721802}  % \textrm{conv4} $0.5 \lunif(t=2) + 1.5 \lalign(\alpha=2)$:
    \\
    \hline
\end{tabular}%
}%
\vspace{-5pt}%
\caption{\nyudepth depth prediction by training a CNN depth regressor from intermediate layer activations. Numbers show mean squared error (MSE) on the validation set. The best result is picked by MSE from \textrm{conv5} layer, among all $64$ encoders trained from scratch with $128$-dimensional output and $128$ batch size.}
\label{tbl:expr_nyudepth}


==> misc/hypersphere/figuretext/experiments/tbl_stl10.tex <==
%auto-ignore
%!TEX root = ../../main.tex

\vspace{-2pt}%
\newcommand{\factor}{0.95}
\resizebox{
  \ifdim\factor\width>\textwidth
    \textwidth
  \else
    \factor\width
  \fi
}{!}{%
\small
\centering
\newcommand{\mroundprec}[1]{\round{#1}{2}\%}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{|c||c||c|c|c|c|}
    \hline
    & Loss Formula
    &  Output + Linear $\uparrow$
    &  Output + $5$-NN $\uparrow$
    &  \textrm{fc7} + Linear $\uparrow$
    &  \textrm{fc7} + $5$-NN $\uparrow$ \\
    \hline\hline

    Best $\lcontr$ only
    & $\lcontr(\tau\narroweq0.1)$ % Loss Formula
    & \mroundprec{77.825} % Linear Output
    & \mroundprec{77.8125} % $5$-NN Output
    & \mroundprec{83.3875} % Linear \textrm{fc7}
    & \mroundprec{75.1875} % $5$-NN \textrm{fc7}
    \\
    \hline

    Best $\lalign$ and $\lunif$ only
    & $\lalign(\alpha\narroweq2) + 0.8 \cdot \lunif(t\narroweq2)$ % Loss Formula
    & \textbf{\mroundprec{81.075}} % Linear Output
    & \textbf{\mroundprec{79.10000000000001}} % $5$-NN Output
    & \textbf{\mroundprec{84.0375}} % Linear \textrm{fc7}
    & \textbf{\mroundprec{76.875}} % $5$-NN \textrm{fc7}
    \\
    \hline

    Best among all encoders
    & $\lalign(\alpha\narroweq2) + 0.8 \cdot \lunif(t\narroweq2)$ % Loss Formula
    & \textbf{\mroundprec{81.075}} % Linear Output
    & \textbf{\mroundprec{79.10000000000001}} % $5$-NN Output
    & \textbf{\mroundprec{84.0375}} % Linear \textrm{fc7}
    & \textbf{\mroundprec{76.875}} % $5$-NN \textrm{fc7}
    \\
    \hline
\end{tabular}%
}%
\vspace{-5pt}%
\caption{\stl classification by a linear or $k$-nearest neighbor ($k$-NN) classifier on encoder output or intermediate layer activations. Numbers show classification accuracies on the validation set. The best result is picked by linear classifier accuracy on encoder outputs, among all $104$ encoders trained from scratch with $128$-dimensional output and $768$ batch size.}
\label{tbl:expr_stl10}


==> misc/hypersphere/text/abstract.tex <==
%auto-ignore
%!TEX root = ../main.tex
% Contrastive representation learning is usually motivated as maximizing the Mutual Information (MI) between the learned encoding and parts of data (\eg, random crops of images \citep{insdis}, next tokens in a sequence \citep{cpc}).
% In this work, we analyze the learned representations from a geometry perspective, quantify the limiting behavior, attempt to provide insights into the standard linear probing evaluation method, and, based on our analysis, provide several tools to improve contrastively learned representations.

Contrastive representation learning has been outstandingly successful in practice.
In this work, we identify two key properties related to the contrastive loss: (1) \emph{alignment} (closeness) of features from positive pairs, and (2) \emph{uniformity} of the induced distribution of the (normalized) features on the hypersphere.
We prove that, asymptotically, the contrastive loss indeed optimizes these properties, and analyze their positive effects on downstream tasks.
Empirically, we introduce an optimizable metric to quantify each property.
Extensive experiments on standard image classification and depth prediction datasets confirm the strong agreement between \emph{both} metrics and downstream task performance. Remarkably, directly optimizing for these two metrics leads to representations with comparable or better performance at downstream tasks than contrastive learning.

==> misc/hypersphere/text/cache.tex <==
%auto-ignore
%!TEX root = ../main.tex
\section{Introduction}

\paragraph{Difference from \citep{saunshi2019theoretical}.} \citep{saunshi2019theoretical} assumes that positive pairs are sampled from the same class, which is often not true in practice. Empirically, since there is no access to the actual labels, the positive pairs are selected as two views of the same data point. Moreover, while \citep{saunshi2019theoretical} make the bounded norm assumption, they do not explain why the assumption is reasonable. Finally, the analysis approaches taken by \citep{saunshi2019theoretical} and our work are essentially different, which may provide different insights.


\section{Motivation}

Standard contrastive loss with $M$ negative samples is
\begin{align}
    & \lc(x, x^+, \{x^-_i\}_{i=1}^M; f, g, \tau) \\
    & \qquad  = - \log \frac{e^{f(x)^T g(x^+) / \tau}}{e^{f(x)^T g(x^+) / \tau} + \sum_{i=1}^M e^{f(x)^T g(x_i^-) / \tau} } \\
    & \qquad  = \log \left( 1 + \sum_{i=1}^M e^{f(x)^T (g(x_i^-) - g(x^+)) / \tau} \right),   \label{eq:contrast}
\end{align}
where the $f(\cdot)$ and $g(\cdot)$ are function mapping data samples to a shared embedding space $R^m$, $\tau$ is the softmax temperature (usually fixed as a hyperparameter).
\footnote{Another common form is using the bilinear critic, i.e., with $f(x) W g(x')^T$ as the exponents (where $W$ is a trainable matrix), which is equivalent with \eqref{eq:contrast} up to an affine transform in the usual case that the output dimensionalities of $f$ and $g$ match. Since the common evaluation methods of learned representation are linear probing (which is what we will investigate) and downstream task performance as input to a neural network (whose first layer is a linear transform) it suffices to discuss the form in \eqref{eq:contrast}.}

Looking at the contrastive loss formula, we see that the loss is encouraging each embedding vector $f(x)$ to be linearly separable with the rest. For finite number of data points, the resulting set of embedding vectors should form a convex polytope with all of them being extreme points.

Does this happen in practice? Figure: yes.

We aim to investigate this observation in principled ways.

In practice, the contrastive loss \eqref{eq:contrast} is optimized over a paired dataset $D = \{(x_i, y_i)\}_{i=1}^N \in (\mathcal{X} \times \mathcal{Y})^N$ of finite size.

We make the following mild assumptions based on empirical practice: \begin{itemize}
    \item In practice, increasing the number of negative samples ($M \rightarrow \infty$) leads to better performance. In this work, we consider the case that of using maximal value $M = N-1$, \ie, contrastive loss of each sample is computed using all other samples as the negatives.
    % \item In practice, the positive pairs $(x, x^+)$ are usually taken as two views of a single data point, \eg, two patches, two channels, two augmented versions, or simply two identical copies.

    % % Notice that the loss in Eq.~\eqref{eq:contrast} admits minimum when

    % To perform analysis in a uniformed setting, we instead only consider the case where the encoder functions $f$ and $g$ operate of the same of copy of a single data point.
    % \begin{align}
    %     & \Lc(x, \{x^-_i\}_{i=1}^N; f, \tau) \\
    %     & \qquad  = - \log \frac{e^{f(x)^T f(x) / \tau}}{e^{f(x)^T f(x) / \tau} + \sum_{i=1}^N e^{f(x)^T f(x_i^-) / \tau} } \\
    %     & \qquad  = \log \left( 1 + \sum_{i=1}^N e^{f(x)^T (f(x_i^-) - f(x)) / \tau} \right),   \label{eq:contrast-simple}
    % \end{align}
    % This could be viewed as a generalization rather than a restriction of the common practice in the sense for each data point \begin{enumerate}
    %     \item construct the positive pair,
    %     \item extract the shared information as the input data to the encoders.
    % \end{enumerate}
\end{itemize}

Therefore, in this work, we consider optimizing the overall loss \begin{equation}
    \Lc(D; f, g, \tau) = \frac{1}{N} \sum_{i=1}^N \lc(x_i, y_i, \{y_j\}_{j\neq i}; f, g, \tau). \label{eq:contrastive-all}
\end{equation}

\subsection{Norm of the embedding}

First, we realize that scaling the embedding vector up often leads to sharper distribution after softmax, and thus lower loss. In practice, we observe this behavior (fixing $\tau$) (1) plot training curve (embedding average norm and loss vs iteration count) and (2) final loss with varying $\tau$.

To illustrate how this behavior could harm embedding quality, we show that under mild assumption, random embeddings can achieve arbitrarily close to a lower bound of \eqref{eq:contrastive-all} simply with scaling.

Recall that our dataset is of the form $D = \{(x_i, y_i)\}_{i=1}^N \in (\mathcal{X} \times \mathcal{Y})^N$.

\begin{theorem}
    For $D$ consisting \iid samples from joint distribution $p(x, y)$ with bounded density function on a continuous domain, the contrastive loss is lower bounded by \begin{equation}
        ....
    \end{equation} With probability $1$, for any $f$ injective over sampled $\{x_i\}_i$ (\ie, $\forall i \neq j, f(x_i) \neq f(x_j)$), there exist a function $g$ \st \begin{equation*}
        \lim_{s \rightarrow \infty} \Lc(D; f, g_s, \tau) - \underbar{$\mathcal{L}$}_\mathsf{contrastive} = 0,
    \end{equation*}
    where $g_s$ is the scaled version of $g$ by a factor of $s$: \begin{equation}
        g_s(y) := s \cdot g(y).
    \end{equation}
\end{theorem}

We define for following quantities representing the frequencies of a certain item appearing in $D$: \begin{itemize}
    \item $c_x = \sum_i 1_{x_i = x}$, for $x \in \mathcal{X}$.
    \item $c_y = \sum_i 1_{y_i = y}$, for $y \in \mathcal{Y}$.
    \item $c_{x,y} = \sum_i 1_{x_i = x \land y_i = y}$, for $(x, y) \in \mathcal{X} \times \mathcal{Y}$.
\end{itemize}

\begin{lemma}
     \eqref{eq:contrastive-all} is lower bounded by \begin{equation}
        \underbar{$\mathcal{L}$}_\mathsf{contrastive} = \frac{1}{N} \sum_i \log c_{x_i} + \log c_{y_i} - \log c_{x_i, y_i}.
    \end{equation}
\end{lemma}
\begin{proof}
    To easily talk about pairs of $D = \{(x_i, y_i\}_{i=1}^N$ that share one or both elements, for $x \in \mathcal{X}$, $y \in \mathcal{Y}$, we define the following index sets: \begin{align*}
        S_x & = \{i \in [N] \colon x_i = x \} \\
        S_y & = \{i \in [N] \colon y_i = y\} \\
        S_{x,y} & = \{i \in [N] \colon (x_i, y_i) = (x, y)\}.
    \end{align*}
    For any $y \in \mathcal{Y}$,
    \begin{align*}
        \lhs \sum_{i \in S_y} \lc(x_i, y_i, \{y_j\}_{j \neq i}; f, g, \tau) \\
        & = \sum_{i \in S_y} \lc(x_i, y, \{y_j\}_{j \neq i}; f, g, \tau) \\
        & = -\sum_{i \in S_y} \log \frac{e^{f(x_i)\T g(y) / \tau}}{\sum_j e^{f(x_i)\T g(y_j) / \tau}} \\
        & \geq -\sum_{i \in S_y}\log
        \frac{e^{f(x_i)\T g(y) / \tau}}{
        \sum_{x \in D_y} \sum_{j \in S_x} e^{f(x_j)\T g(y) / \tau}} \\
        & = -\sum_{i \in S_y}\log
        \frac{e^{f(x_i)\T g(y) / \tau}}{
        \sum_{x \in D_y} c_x e^{f(x_j)\T g(y) / \tau}} \\
        & \geq \min_{\alpha_x \colon x \in D_y, \sum_{x \in D_x} \alpha_x=1} -\sum_{i \in S_y}\log \frac{\alpha_{x_i}}{c_{x_i}} \\
        & = \min_{\alpha_x \colon x \in D_y, \sum_{x \in D_x} \alpha_x=1} -\sum_{x \in D_y} c_{x,y} \log \frac{\alpha_{x}}{c_{x}} \\
        & = \sum_{x \in D_y} c_{x,y} \log \frac{c_{x} c_{y}}{c_{x,y}}
    \end{align*}
\end{proof}

% \begin{theorem}
%     If $\max_{y \in \mathcal{Y}} c_Y(y_i) < m$, then with probability $1$, for \iid $u_i \sim \mathcal{U}(\sphere^{m-1})$, $i = 1, \dots, N$, for the following encoder defined as \begin{equation*}
%         f_s(x_i) = s \cdot u_i, \quad s \in \R,
%     \end{equation*}
%     there exist a function $g$ \st \begin{equation*}
%         \lim_{s \rightarrow \infty} \Lc(D; f_s, g, \tau) - \underbar{$\mathcal{L}$}_\mathsf{contrastive} = 0.
%     \end{equation*}
% \end{theorem}

% \begin{proof}
%     Let $\sigma^m$ be the normalized area measure on $\sphere^m$, which is also a probability measure.

%     Since $\max_{y \in \mathcal{Y}} c_Y(y_i) < m$, for any $y \in \mathcal{Y}$, $\size{S_y} < m$ and the spherical convex hull formed by $\{u_i \colon i \in S_y\}$ has $\sigma^m$ measure $0$.
% \end{proof}

In other words,
% To explain this, we prove the following theorem:
% \begin{theorem}
%     Consider embeddings $x = \{x_i\}_{i=1,\dots N}$, $R > 0$,
%     \begin{equation}
%         \min_{x \colon \norm{x_i} \leq R \forall i} \sum_i \log \frac{}{}
%     \end{equation}
% \end{theorem}

\begin{theorem}
    Consider paired dataset $D = \{(x_i, y_i)\}_{i=1}^N \in (\mathcal{X} \times \mathcal{Y})^N$, measurable functions $f \colon \mathcal{X} \rightarrow \sphere^m$ and $g \colon \mathcal{Y} \rightarrow \sphere^m$, we have \begin{align*}
        \mathcal{L}_\mathsf{max\_margin}(D; f, g, \tau)
        & \leq \Lc(D; f, g, \tau) \\
        & \leq c \wcdot \mathcal{L}_\mathsf{max\_margin}(D; f, g, \tau) + b,
    \end{align*}
    for the max pairwise distance loss \begin{equation*}
        \mathcal{L}_\mathsf{max\_dist}(D; f, g, \tau) = \frac{1}{\tau N} \sum_{i \neq j} \norm{f(x_i) - g(y_j)}_2^2,
    \end{equation*}
    the alignment loss \begin{equation*}
        \mathcal{L}_\mathsf{align}(D; f, g, \tau) = \frac{1}{\tau N} \sum_{i \neq j} \norm{f(x_i) - g(y_j)}_2^2,
    \end{equation*}
    and some constant $c \in \R_+$ and $b \in \R$ only depending on $N$ and $\tau$.
\end{theorem}

\begin{proof}
    For simplicity, we overload and define the notation $f_i = f(x_i)$ and $g_i = g(y_i)$.

    \begin{align*}
        & \Lc(D; f, g, \tau)\\
        & = \frac{1}{N} \sum_i \log(1 + \sum_{j \neq i} \exp( \frac{(f_j - f_i)\T g_i}{\tau} )) \\
        & \geq\frac{1}{N} \sum_i \max(0, \max_{j\neq i} \frac{(f_j - f_i)\T g_i}{\tau}) \\
        & \geq \frac{1}{N} \sum_i \log(1 + (N-1) \exp(\frac{1}{N - 1} \sum_{j \neq i} \frac{(f_j - f_i)\T g_i}{\tau} )) \\
        & = \frac{1}{N} \sum_i \log(1 + \exp(\frac{\log (N-1)}{N-1} \sum_{j \neq i} \frac{(f_j - f_i)\T g_i}{\tau} )) \\
        & \geq \frac{\log (N-1)}{N (N-1)} \sum_i \max(0, \sum_{j \neq i} \frac{(f_j - f_i)\T g_i}{\tau}) \\
        & = \frac{\log N}{\tau N^2} \sum_{i \neq j} f_j\T g_i - f_i\T g_i \\
        & = \frac{\log N}{\tau N^2} \sum_{i \neq j} \norm{f_i - g_i}_2^2 - \norm{f_j - g_i}_2^2 \\
        & = \frac{(N-1)\log N}{\tau N} \sum_i \norm{f_i - g_i}_2^2 - \frac{\log N}{\tau N^2} \sum_{i \neq j} \norm{f_j - g_i}_2^2 \\
        & = \frac{N-1}{N} \frac{\log N}{\tau} \bigg(
        \underbrace{\sum_i \norm{f_i - g_i}_2^2}_{\text{alignment between $f$ and $g$}} -
        \underbrace{\frac{1}{N (N-1)} \sum_{i \neq j} \norm{f_j - g_i}_2^2}_{\text{pairwise distances among embeddings}}
        \bigg) \\
    \end{align*}

    % \begin{align*}
    %     & \Lc(D; f, g, \tau)\\
    %     & = \frac{1}{N} \sum_i \log(1 + \sum_{j \neq i} \exp( \frac{(f_j - f_i)\T g_i}{\tau} )) \\
    %     & \geq \frac{1}{N} \sum_i \log(1 + (N-1) \exp(\frac{1}{N - 1} \sum_{j \neq i} \frac{(f_j - f_i)\T g_i}{\tau} )) \\
    %     & = \frac{1}{N} \sum_i \log(1 + \exp(\frac{\log (N-1)}{N-1} \sum_{j \neq i} \frac{(f_j - f_i)\T g_i}{\tau} )) \\
    %     & \geq \frac{\log (N-1)}{N (N-1)} \sum_i \max(0, \sum_{j \neq i} \frac{(f_j - f_i)\T g_i}{\tau}) \\
    %     & = \frac{\log N}{\tau N^2} \sum_{i \neq j} f_j\T g_i - f_i\T g_i \\
    %     & = \frac{\log N}{\tau N^2} \sum_{i \neq j} \norm{f_i - g_i}_2^2 - \norm{f_j - g_i}_2^2 \\
    %     & = \frac{(N-1)\log N}{\tau N} \sum_i \norm{f_i - g_i}_2^2 - \frac{\log N}{\tau N^2} \sum_{i \neq j} \norm{f_j - g_i}_2^2 \\
    %     & = \frac{N-1}{N} \frac{\log N}{\tau} \bigg(
    %     \underbrace{\sum_i \norm{f_i - g_i}_2^2}_{\text{alignment between $f$ and $g$}} -
    %     \underbrace{\frac{1}{N (N-1)} \sum_{i \neq j} \norm{f_j - g_i}_2^2}_{\text{pairwise distances among embeddings}}
    %     \bigg) \\
    % \end{align*}

    % \begin{align*}
    %     \Lc(D; f, g, \tau)
    %     & = \frac{1}{N} \sum_i \log(1 + \sum_{j \neq i} \exp( \frac{(f_j - f_i)\T g_i}{\tau} )) \\
    %     & \geq \frac{1}{N} \sum_i \log(1 + \max_{j \neq i} \exp( \frac{(f_j - f_i)\T g_i}{\tau} )) \\
    %     & = \frac{1}{N} \sum_i \log(1 + \exp( \frac{ (\max_{j \neq i} f_j\T g_i) - f_i\T g_i}{\tau} )) \\
    %     & \geq \frac{1}{N\tau} \sum_i (\max_{j \neq i} f_j\T g_i) - f_i\T g_i \\
    %     & \geq \frac{1}{N\tau} \sum_i (\max_{j \neq i} f_j\T g_i) - 2 \\
    %     & = - \frac{1}{N\tau} \sum_i (\max_{j \neq i} f_j\T g_i) - 2 \\
    %     & \geq \frac{1}{N\tau} \max_{i\neq j} f_j\T g_i - f_i\T g_i \\
    %     & = \mathcal{L}_\mathsf{max\_margin}(D; f, g, \tau).
    % \end{align*}

    % Consider the strictly convex and strictly monotonically increasing function $l(x) = \log(1 + (N - 1) \exp \frac{x}{\tau})$ and its best linear upper bound over $[-1, 1]$: \begin{align*}
    %     \bar{l}(x)
    %     & = \frac{l(1) - l(-1)}{2} \frac{x + 1}{2} + l(-1) \\
    %     & = \frac{l(1) - l(-1)}{4} x + \frac{l(1) + 3 l(-1)}{4} \\
    %     & = \frac{l(1) - l(-1)}{4} x + \frac{l(1) + 3 l(-1)}{4}.
    % \end{align*}

    % \begin{align*}
    %     \Lc(D; f, g, \tau)
    %     & = \sum_i \log(1 + \sum_{j \neq i} \exp( \frac{(f_j - f_i)\T g_i}{\tau} )) \\
    %     & = \sum_i \log(1 + (N-1) \exp( \frac{ (\max_{j \neq i} f_j\T g_i) - f_i\T g_i}{\tau} )) \\
    %     & = \sum_i l( (\max_{j \neq i} f_j\T g_i) - f_i\T g_i ) \\
    %     & \leq N l( (\max_{j \neq i} f_j\T g_i) - f_i\T g_i ) \\
    %     & \leq N \bar{l}( (\max_{j \neq i} f_j\T g_i) - f_i\T g_i ) \\
    %     & = N \frac{l(1) - l(-1)}{4} \left( (\max_{j \neq i} f_j\T g_i) - f_i\T g_i \right) + \frac{l(1) + 3 l(-1)}{4} \\
    %     & = \mathcal{L}_\mathsf{max\_margin}(D; f, g, \tau).
    % \end{align*}

    Since $\mathtt{LogSumExp}$ is convex and monotonically increasing, so is $l(x_1, \dots, x_{N-1}) = \log (1 + \sum_j \exp \frac{x_j}{\tau})$, which can be crudely bounded above by the linear function over $[-2, 2]^{N-1}$ \begin{align*}
        \bar{l}(x_1, \dots, x_{N-1})
        & = l(-2, \dots, -2) + \\
        & \qquad \frac{1}{4} \left(\sum_j x_j+2 \right) \left(l(2, -2, \dots, -2) - l(-2, \dots, -2) \right) \\
        & = \frac{N-1}{2} l(2, -2, \dots, -2) - \frac{N-3}{2} l(-2, \dots, -2) + \\
        & \qquad \frac{l(2, -2, \dots, -2) - l(-2, \dots, -2)}{4} \sum_j x_j \\
        & = \log (1+(N-1) e^{-2/\tau}) + \\
        & \qquad (\frac{N-1}{2} + \frac{\sum_j x_j}{4}) \log \left( 1 + \frac{e^{2/\tau} - e^{-2/\tau}}{1+(N-1) e^{-2/\tau}} \right).
    \end{align*} This can be easily shown by realizing $\frac{\partial \log (a + e^x)}{\partial x} = \frac{e^x}{a + e^x}$ is a decreasing function \wrt $a$ for fixed $x$.


    \begin{align*}
        \Lc(D; f, g, \tau)
        & = \frac{1}{N} \sum_i \log(1 + \sum_{j \neq i} \exp( \frac{(f_j - f_i)\T g_i}{\tau} )) \\
        & = \frac{1}{N} \sum_i l(f_1, \dots, f_{i-1}, f_{i+1}, \dots, f_N) \\
        & \leq \frac{1}{N} \sum_i \bar{l}(f_1, \dots, f_{i-1}, f_{i+1}, \dots, f_N) \\
        & = \log (1+(N-1) e^{-2/\tau}) + \\
        & \qquad (\frac{N-1}{2} + \frac{\sum_{i \neq j} (f_j - f_i)\T g_i}{4N}) \log \left( 1 + \frac{e^{2/\tau} - e^{-2/\tau}}{1+(N-1) e^{-2/\tau}} \right) \\
        & = N l(-2, \dots, -2) + \frac{1}{4} \left(\sum_{i \neq j} (f_j - f_i)\T g_i +2 \right) \left(l(2, -2, \dots, -2) - l(-2, \dots, -2) \right) \\
        & = \mathcal{L}_\mathsf{max\_margin}(D; f, g, \tau).
    \end{align*}

    Alternatively, with probability 1,
    \begin{align*}
        \min_g \Lc(D; f, g, \tau)
        & = \min_g \frac{1}{N} \sum_i \log(\sum_{j} \exp( \frac{(f_j - f_i)\T g_i}{\tau} )) \\
        & \leq \frac{1}{N} \sum_i \log(\sum_{j} \exp( \frac{(f_j - f_i)\T f_i}{\tau} )) \\
        & = \frac{1}{N} \log \prod_i \sum_{j} \exp( \frac{f_j \T f_i - 1}{\tau} ) \\
        & = \frac{1}{N} \log \sum_{\pi \in [N]^N} \prod_j \exp( \frac{f_j \T f_{\pi_j} - 1}{\tau} ) \\
        & = \frac{1}{N} \log \sum_{\pi \in [N]^N} \exp( \sum_j \frac{f_j \T f_{\pi_j} - 1}{\tau} ) \\
        & = \frac{\log \sum_{i} \binom{N}{i} \log i}{N \tau}  \left (\max_{k \neq l}  f_{k} \T f_{l} - 1 \right).  \\
    \end{align*}

\end{proof}

==> misc/hypersphere/text/discussion.tex <==
%auto-ignore
%!TEX root = ../main.tex

\emph{Alignment} and \emph{uniformity} are often alluded to as motivations for representation learning methods (see Figure~\ref{fig:align_unif}). However, a thorough understanding of these properties is lacking in literature.

Are they in fact related to the representation learning methods? Do they actually agree with the representation quality (measured by downstream task performance)?

In this work, we have presented a detailed investigation on the relation between these properties and the popular paradigm of contrastive representation learning. Through theoretical analysis and extensive experiments, we are able to relate the contrastive loss with the alignment and uniformity properties, and confirm their strong connection with downstream task performances. Remarkably, we have revealed that directly optimizing our proposed metrics often leads to representations of better quality.

Below we summarize several suggestions for future work.

\paragraph{Niceness of the unit hypersphere.} Our analysis was based on the empirical observation that representations are often $\ell_2$ normalized. Existing works have motivated this choice from a manifold mapping perspective \citep{liu2017sphereface,s-vae18} and computation stability \citep{xu2018spherical,wang2017normface}. However, to our best knowledge, the question of why the unit hypersphere is a nice feature space is not yet rigorously answered. One possible direction is to formalize the intuition that connected sets with smooth boundaries are nearly linearly separable in the hyperspherical geometry (see Figure~\ref{fig:hypersphere_linsep}), since linear separability is one of the most widely used criterion for representation quality and is related to the notion of disentanglement.

\paragraph{Beyond contrastive learning.} Our analysis focused on the relationship between contrastive learning and the alignment and uniformity properties on the unit hypersphere. However, the ubiquitous presence of $\ell_2$ normalization in the representation learning literature suggests that the connection may be more general. In fact, several existing empirical methods are directly related to uniformity on the hypersphere \citep{bojanowski2017unsupervised,s-vae18,xu2018spherical}. We believe that relating a broader class of representations to uniformity and/or alignment on the hypersphere will provide novel insights and lead to better empirical algorithms.


==> misc/hypersphere/text/distribution.tex <==
%auto-ignore
%!TEX root = ../main.tex

\input{figuretext/distribution/toy2d}

The contrastive loss encourages learned feature representation for positive pairs to be similar, while pushing features from the randomly sampled negative pairs apart. Conventional wisdom says that representations should extract the most shared information between positive pairs and remain invariant to other noise factors \citep{linsker1988self,tian2019contrastive,wu2020importance,bachman2019learning}. Therefore, the loss should prefer two following properties: \begin{itemize}
    \item \emph{Alignment}: two features from a positive pair should be close to each other, and thus invariant to noise factors.
    \item \emph{Uniformity}: feature vectors should be roughly uniformly distributed on the unit hypersphere $\sphere^{m-1}$, preserving as much information as possible.
\end{itemize}

To empirically verify this, we visualize \cifar \citep{torralba200880,krizhevsky2009learning} representations on $\sphere^1$ ($m = 2$) obtained via three different methods: \begin{itemize}
    \item Random initialization.
    \item Supervised predictive learning: An encoder and a linear classifier are jointly trained from scratch with cross entropy loss on supervised labels.
    \item Unsupervised contrastive learning: An encoder is trained according to $\lcontr$ with $\tau = 0.5$ and $M = 256$.
\end{itemize} All three encoders share the same AlexNet based architecture \citep{krizhevsky2012imagenet}, modified to map input images to 2D vectors in $\sphere^1$. Both predictive and contrastive learning use standard data augmentations to augment the dataset / sample positive pairs.

Figure~\ref{fig:toy2d} summarizes the resulting distributions of validation set features. Indeed, features from unsupervised contrastive learning (bottom in Figure~\ref{fig:toy2d}) exhibit the most uniform distribution, and are closely clustered for positive pairs.

The form of the contrastive loss in Eqn.~\eqref{eq:contrastive_loss} also suggests this. We present informal arguments below, followed by more formal treatment in Section~\ref{sec:limit}. From the symmetry of $p$, we can derive%
\begin{equation*}
\begin{split}
    & \lcontr(f; \tau, N) = \expectunder[(x, y) \sim \distnpos]{- f(x)\T f(y) / \tau} \\
    % & = \expect[\substack{
    % (x, y) \sim p \\
    % \{x^-_i\}_{i=1}^{N} \iidsim D
    % }]{- \log \frac{e^{f(x)\T f(y) / \tau}}{e^{f(x)\T f(y) / \tau} + \sum_i e^{f(x^-_i)\T f(y) / \tau}}} \\
    % & = \expectunder{- f(x)\T f(y) / \tau}  +
    % \expectunder{\log \left( e^{f(x)\T f(y) / \tau} + \sum_i e^{f(x^-_i)\T f(y) / \tau} \right)} \\
    % & \qquad  + \\
    & \quad +\hspace{-5pt}\expectundernear[\substack{
    (x, y) \sim \distnpos \\
    \{x^-_i\}_{i=1}^{N} \iidsim \distndata
    }]{\log\hspace{-2pt}\left( e^{f(x)\T f(y) / \tau}+ \sum_i e^{f(x^-_i)\T f(x) / \tau} \right)}.
\end{split}
\end{equation*}
Because the $\sum_i e^{f(x^-_i)\T f(x) / \tau}$ term is always positive and bounded below, the loss favors smaller $\expect{- f(x)\T f(y) / \tau}$, \ie, having more aligned positive pair features. Suppose the encoder is perfectly aligned, \ie, $\prob{f(x) = f(y)} = 1$, then minimizing the loss is equivalent to optimizing \begin{equation*}
    \expectunder[\substack{
    x \sim \distndata \\
    \{x^-_i\}_{i=1}^{N} \iidsim \distndata
    }]{\log \left( e^{1 / \tau}+ \sum_i e^{f(x^-_i)\T f(x) / \tau} \right)},
\end{equation*}
which is akin to maximizing pairwise distances. Intuitively, pushing all features away from each other should indeed cause them to be roughly uniformly distributed.

\input{text/metric}
\input{text/theory}
% \input{text/niceness}

==> misc/hypersphere/text/experiments.tex <==
%auto-ignore
%!TEX root = ../main.tex

\input{figuretext/experiments/scatter}

In this section, we empirically verify the hypothesis that alignment and uniformity are desired properties for representations. Recall that our two metrics are \begin{align*}
\if\fixsubmission1
    \lalign(f; \alpha) & \trieq - \expect[(x, y) \sim \distnpos] {\norm{f(x) - f(y)}_2^\alpha} \\
\else
    \lalign(f; \alpha) & \trieq \expect[(x, y) \sim \distnpos] {\norm{f(x) - f(y)}_2^\alpha} \\
\fi
    \lunif(f; t) & \trieq \log~\expect[x, y \iidsim \distndata] {e^{-t \norm{f(x) - f(y)}_2^2}}.
\end{align*}\if\fixsubmission0\vspace{-15pt}\fi

We conduct extensive experiments with convolutional neural network (CNN) based encoders on two popular representation learning benchmarks with distinct types of downstream tasks: \begin{itemize}
    \item \stl \citep{coates2011stl10} classification on encoder outputs or intermediate activations with a linear or $k$-nearest neighbor ($k$-NN) classifier.
    \item \nyudepth \citep{Silberman:ECCV12} depth prediction on encoder intermediate activations after convolution layers.
\end{itemize}
We follow the standard practice and choose the positive pairs as two independent augmentations of the same image. Encoders are optimized using minibatch stochastic gradient descent for all experiments. For $\lcontr$, negatives are other samples within the minibatch. For $\lunif$, we optimize the logarithm of average pairwise feature potentials also within the minibatch.

See supplementary material for more experiment details.

% \subsection{Correlation with Downstream Task Performance}

\begin{table*}[t!]%
    \centering
    \input{figuretext/experiments/tbl_stl10}
\end{table*}
\begin{table*}[t!]%
    \centering
    \input{figuretext/experiments/tbl_nyudepth}
\end{table*}

We train a total of $260$ \stl encoders and $64$ \nyudepth encoders without supervision. The encoders are optimized \wrt weighted combinations of $\lcontr$, $\lalign$, and/or $\lunif$, with varying \begin{itemize}
    \item (possibly zero) weights on the three losses,
    \item temperature $\tau$ for $\lcontr$,
    \item $\alpha \in \{1, 2\}$ for $\lalign$, fixed $t = 2$ for $\lunif$,
    \item number of training epochs,
    \item learning rate,
    \item batch size (affecting the number of (negative) pairs for $\lcontr$ and $\lunif$),
    \item embedding dimension,
    \item initialization (from scratch vs.~a pretrained encoder).
\end{itemize}
See supplementary material for the exact combinations.

\paragraph{$\lalign$ and $\lunif$ strongly agree with downstream task performance.}
For each encoder, we measure the downstream task performance, and the $\lalign$, $\lunif$ metrics on the validation set. Figure~\ref{fig:expr_scatter} visualizes the trends between both metrics and representation quality. We observe that the two metrics strongly agrees the representation quality overall. In particular, the best performing encoders are exactly the ones with low $\lalign$ and $\lunif$, \ie, the lower left corners in Figure~\ref{fig:expr_scatter}.

\input{figuretext/experiments/finetune}
\input{figuretext/experiments/lgda_trend}

\paragraph{Directly optimizing only $\lalign$ and $\lunif$ can lead to better representations.}
As shown in Table~\ref{tbl:expr_stl10} and Table~\ref{tbl:expr_nyudepth}, the best performing encoder is consistently the one trained with only $\lalign(\alpha\narroweq2)$ and $\lunif(t\narroweq2)$ for both tasks. Theoretically, Theorem~\ref{thm:asym_inf_negatives} showed that $\lcontr$ optimizes alignment and uniformity asymptotically with infinite negative samples. This empirical performance gap suggests that directly optimizing these properties can be superior in practice, when we can only have finite negatives.

\paragraph{Both alignment and uniformity are necessary for a good representation. }
Figure~\ref{fig:expr_lgda_trend} shows how the final encoder changes in response to optimizing differently weighted combinations of $\lalign$ and $\lunif$ on \stl. The trade-off between the $\lalign$ and $\lunif$ indicates that perfect alignment and perfect uniformity are likely hard to simultaneously achieve in practice. However, the inverted-U-shaped accuracy curve confirms that both properties are indeed necessary for a good encoder.
When $\lalign$ is weighted much higher than $\lunif$, degenerate solution occurs and all inputs are mapped to the same feature vector ($\exp \lunif = 1)$. However, as long as the ratio between two weights is not too large (\eg, $< 10$), we observe that the representation quality remains relatively good and insensitive to the exact weight choices.

% \subsection{Causation on Downstream Task Performance}


\paragraph{$\lalign$ and $\lunif$ causally affect downstream task performance.} We take an encoder trained with $\lcontr$ using a suboptimal temperature $\tau = 2.5$, and finetune it according to $\lalign$ and/or $\lunif$. Figure~\ref{fig:expr_finetune} visualizes the finetuning trajectories. When only one of alignment and uniformity is optimized, the corresponding metric improves, but both the other metric and performance degrade. However, when both properties are optimized, the representation quality steadily increases. These trends confirm the causal effect of alignment and uniformity on the representation quality, and suggest that directly optimizing them can be a reasonable choice.


==> misc/hypersphere/text/introduction.tex <==
%auto-ignore
%!TEX root = ../main.tex

A vast number of recent empirical works learn representations with a unit $\ell_2$ norm constraint, effectively restricting the output space to the unit hypersphere \citep{parkhi2015deep,schroff2015facenet,liu2017sphereface,hasnat2017mises,wang2017normface,bojanowski2017unsupervised,mettes2019hyperspherical,hou2019learning,s-vae18,xu2018spherical}, including many recent unsupervised contrastive representation learning methods \citep{wu2018unsupervised,bachman2019learning,tian2019contrastive,he2019momentum}.

Intuitively, having the features live on the unit hypersphere leads to several desirable traits.
% \todo{replace with ``coordinate less ness'', and necessity of normalization }
Fixed-norm vectors are known to improve training stability in modern machine learning where dot products are ubiquitous \citep{xu2018spherical,wang2017normface}. Moreover, if features of a class are clustered together, they naturally are nearly linearly separable with the rest of the feature space (see Figure~\ref{fig:hypersphere_linsep}), a common criterion used to evaluate representation quality.

\begin{figure}[t]
    \centering\vspace{-8pt}
    \begin{subfigure}[b]{\linewidth}
    \centering
    \captionsetup{justification=centering}
    \includegraphics[page=2, width=0.88\linewidth, trim=500 180 500 200, clip]{figures/intuition.pdf}\vspace{-5pt}
    \caption*{\textbf{Alignment: }Similar samples have similar features.\\(Figure inspired by \citet{tian2019contrastive}.)}%\vspace{-1pt}
    \end{subfigure}
    \begin{subfigure}[b]{\linewidth}
    \centering
    \captionsetup{justification=centering}
    \includegraphics[page=3, width=0.88\linewidth, trim=500 220 500 230, clip]{figures/intuition.pdf}\vspace{-5pt}
    \caption*{\textbf{Uniformity: }Preserve maximal information.}
    \end{subfigure}\vspace{-3pt}
    \caption{Illustration of alignment and uniformity of feature distributions on the output unit hypersphere. \stl \citep{coates2011stl10} images are used for demonstration.} \label{fig:align_unif}
\end{figure}


\begin{figure}
    \centering\vspace{-3pt}%\vspace{-50pt}
    \includegraphics[page=1, width=0.9\linewidth, trim=450 160 450 85, clip]{figures/intuition.pdf}\vspace{-10pt}
    \caption{\textbf{Hypersphere: }When classes are well-clustered on the hypersphere (forming spherical caps), they are linearly separable. The same does not hold for Euclidean spaces.
    % If features from a class correspond to a connected compact set with smooth boundary on the hypersphere, they are nearly linearly separable with the rest of the feature space.
    } \label{fig:hypersphere_linsep}
\end{figure}

While the unit hypersphere is a popular choice of feature space, not all encoders that map onto it are created equal. Additionally, recent works argue that representations should be invariant to unnecessary details, and preserve as much information as possible \citep{oord2018representation,tian2019contrastive,hjelm2018learning,bachman2019learning}. Let us call these two properties \emph{alignment} and \emph{uniformity} (see Figure~\ref{fig:align_unif}). \emph{Alignment} favors encoders that assign similar features to similar samples. \emph{Uniformity} prefers maximal entropy feature distribution, \ie, the uniform distribution on the unit hypersphere.

In this work, we analyze the \emph{alignment} and \emph{uniformity} properties. We show that the popular unsupervised contrastive representation learning in fact directly optimizes for these two properties in the limit of infinite negative samples. Empirically, we propose theoretically-motivated metrics for alignment and uniformity, and observe strong agreement between them and downstream task performance. Remarkably, directly optimizing for these two metrics leads to comparable or better performance than contrastive learning.

Our main contributions are:
\begin{itemize}
    \item We propose qantifiable metrics for \emph{alignment} and \emph{uniformity} as two measures of representation quality, with theoretical motivations.
    \item We prove that the contrastive loss optimizes for alignment and uniformity asymptotically.
    \item Empirically, we find strong agreement between \emph{both} metrics and downstream task performance.
    \item Despite being simple in form, our proposed metrics, when directly optimized with no other loss, empirically lead to comparable or better performance at downstream tasks than contrastive learning.
\end{itemize}

% 1. people learn representation on hypersphere
% 2. uniformity and alignment are nice properties (figure, explain)
% 3. the popular contrastive loss turns out optimizing them asymptotically
% 4. empirical results: they correlates nicely, direct optimizing gives better results,

==> misc/hypersphere/text/metric.tex <==
%auto-ignore
%!TEX root = ../main.tex

\subsection{Quantifying Alignment and Uniformity} \label{sec:unif-align}

For further analysis, we need a way to measure alignment and uniformity. We propose the following two metrics (losses).

\subsubsection{Alignment}
The alignment loss is straightforwardly defined with the expected distance between positive pairs:  %
\if\fixsubmission1
\begin{equation*}
    \lalign(f; \alpha) \trieq - \expectunder[(x, y) \sim \distnpos] {\norm{f(x) - f(y)}_2^\alpha}, \quad \alpha > 0.
\end{equation*}
\else
\begin{equation*}
    \lalign(f; \alpha) \trieq \expectunder[(x, y) \sim \distnpos] {\norm{f(x) - f(y)}_2^\alpha}, \quad \alpha > 0.
\end{equation*}
\fi

\input{figuretext/distribution/gaussian_vis}

\subsubsection{Uniformity}
We want the uniformity metric to be both asymptotically correct (\ie, the distribution optimizing this metric should converge to uniform distribution) and empirically reasonable with finite number of points. To this end, we consider the Gaussian potential kernel (also known as the Radial Basis Function (RBF) kernel) $G_t \colon \sphere^{d} \times \sphere^{d} \rightarrow \R_+$ \citep{cohn2007universally,borodachov2019discrete}: \begin{equation*}
    G_t(u, v) \trieq e^{-t \norm{u - v}_2^2} = e^{2t \cdot u\T v - 2t}, \quad t > 0,
\end{equation*}
and define the uniformity loss as the logarithm of the average pairwise Gaussian potential: \begin{align*}
    \lunif(f; t)
    & \trieq \log \expectunder[x, y \iidsim \distndata] {G_t(u, v)} \\
    & = \log \expectunder[x, y \iidsim \distndata] {e^{-t \norm{f(x) - f(y)}_2^2}}, \quad t > 0,
\end{align*}
where $t$ is a fixed parameter.

The average pairwise Gaussian potential is nicely tied with the uniform distribution on the unit hypersphere.

\begin{definition}[Uniform distribution on $\sphere^{d}$]
    $\sigma_{d}$ denotes the normalized surface area measure on $\sphere^{d}$.
\end{definition}

First, we show that the uniform distribution is the unique distribution that minimize the expected pairwise potential.
\begin{proposition}
    For $\mathcal{M}(\sphere^{d})$ the set of Borel probability measures on $\sphere^{d}$, $\sigma_{d}$ is the unique solution of \begin{equation*}
        \min_{\mu \in \mathcal{M}(\sphere^{d})} \int_u \int_v G_t(u, v) \diff \mu \diff \mu.
    \end{equation*}
\end{proposition}
\begin{proof}
    See supplementary material.
\end{proof}

In addition, as number of points goes to infinity, distributions of points minimizing the average pairwise potential converge weak$^*$ to the uniform distribution. Recall the definition of the weak$^*$ convergence of measures.

\begin{definition}[Weak$^*$ convergence of measures]
    A sequence of Borel measures $\{\mu_n\}_{n=1}^\infty$ in $\R^p$ converges weak$^*$ to a Borel measure $\mu$ if for all continuous function $f \colon \R^p \rightarrow \R$, we have \begin{equation*}
        \lim_{n\rightarrow \infty} \int f(x) \diff \mu_n(x) = \int f(x) \diff \mu(x).
    \end{equation*}
    % In this case, we write $\mu_n \weakconv \mu$.
\end{definition}

\begin{proposition}
    For each $N > 0$, the $N$ point minimizer of the average pairwise potential is \begin{equation*}
        \mathbf{u}^*_N = \argmin_{u_1, u_2, \dots, u_N \in \sphere^{d}} \sum_{1 \leq i < j \leq N} G_t(u_i, u_j).
    \end{equation*}
    The normalized counting measures associated with the $\{\mathbf{u}^*_N\}_{N=1}^\infty$ sequence converge weak$^*$ to $\sigma_d$.
\end{proposition}
\begin{proof}
    See supplementary material.
\end{proof}

Empirically, we evaluate the average pairwise potential of various finite point collections on $\sphere^1$ in Figure~\ref{fig:gaussian_vis}. The values nicely align with our intuitive understanding of uniformity. %\todo{add higher dim trend plot}

==> misc/hypersphere/text/niceness.tex <==
%auto-ignore
%!TEX root = ../main.tex


\subsection{Why are Uniformity and Alignment Nice?}
\todo{intuition, motivate with class-positive-pair examples, maybe theory}

But why are uniformity and alignment nice properties?

\subsubsection{$\ppos$ and Alignment Affect Class Concentration}

First, we observe hat class concentration naturally happens in unsupervised contrastive learning (\eg, in Figure~\ref{fig:toy2d}), \ie, samples of the same class are mapped to nearby feature vectors.

Some may argue that this is the result of the powerful inductive bias of convolutional neural network (CNN) encoder \citep{cohen2016inductive}. We will show below that the choice of $p_\mathsf{pos}$ and the alignment property also empirically play important roles.

Analogous to $\lalign$, we use the following metric to quantify class concentration. For a label distribution $\pcls$, \begin{equation}
    \lclscon(f) \trieq - \expectunder[c \sim \pcls] {\expectunder[x, y \iidsim \distndata(\cdot \given c)] {\norm{f(x) - f(y)}_2^2}}.%, \quad \alpha > 0.
\end{equation}%
\Ie, the expectation is now taken over sample pairs that share the same class label.

To investigate the effect of $\ppos$ and alignment, we consider four different $\ppos$ choices: \begin{itemize}
    \item Light augmentation: \todo{talk about how this violates matching marginal?}%$\ppos(x, y) = \indic{x = y} \pdata(x)$.
    \item Normal augmentation:
    \item Normal augmentation + sampling from same class.
\end{itemize}
and encoders trained in three different ways: \begin{itemize}
    \item Supervised predictive learning. \todo{fix desc}
    \item Unsupervised contrastive learning with various temperature.
    \item Unsupervised $\lalign$ and $\lunif$ learning with various weights.
\end{itemize}

\todo{talk about class concentration, latent class, relation with alignment}

\subsubsection{Sets on the Hypersphere and Linear Separability}



\todo{visualization of uniform, class, linear separability}

==> misc/hypersphere/text/preliminaries.tex <==
%auto-ignore
%!TEX root = ../main.tex

The popular unsupervised contrastive representation learning method (often referred to as \emph{contrastive learning} in this paper) learns representations from unlabeled data. It assumes a way to sample \emph{positive pairs}, representing similar samples that should have similar representations. Empirically, the positive pairs are often obtained by taking two independently randomly augmented versions of the same sample, \eg two crops of the same image \citep{wu2018unsupervised,hjelm2018learning,bachman2019learning,he2019momentum}.

Let $\distndata(\cdot)$ be the data distribution over $\R^n$ and $\distnpos(\cdot, \cdot)$ the distribution of positive pairs over $\R^n \times \R^n$. Based on empirical practices, we assume the following property.

\begin{assumption}
    Distributions $\distndata$ and $\distnpos$ should satisfy%
    \begin{itemize}
        \item Symmetry: $\forall x, y,~ \distnpos(x, y) = \distnpos(y, x)$.
        \item Matching marginal: $\forall x,~ \int \distnpos(x, y) \diff y = \distndata(x)$.
    \end{itemize}
\end{assumption}

We consider the following specific and widely popular form of contrastive loss for training an encoder $f \colon \R^n \rightarrow \sphere^{m-1}$, mapping data to $\ell_2$ normalized feature vectors of dimension $m$. This loss has been shown effective by many recent representation learning methods \citep{logeswaran2018efficient,wu2018unsupervised,tian2019contrastive,he2019momentum,hjelm2018learning,bachman2019learning}.
\begin{equation}
\begin{split}
    & \lcontr(f; \tau, M) \trieq \\
    & \quad \expectunder[\substack{
        (x, y) \sim \distnpos \\
        \{x^-_i\}_{i=1}^M \iidsim \distndata
    }]{- \log \frac{e^{f(x)\T f(y) / \tau}}{e^{f(x)\T f(y) / \tau} + \sum_i e^{f(x^-_i)\T f(y) / \tau}}},
\end{split} \label{eq:contrastive_loss}
\end{equation}
where $\tau > 0$ is a scalar temperature hyperparameter, and $M \in \Z_+$ is a fixed number of negative samples.

\paragraph{Necessity of normalization.} Without the norm contraint, the softmax distribution can be made arbitrarily sharp by simply scaling all the features. \citet{wang2017normface} provided an analysis on this effect and argued for the necessity of normalization when using feature vector dot products in a cross entropy loss, as is in Eqn.~\eqref{eq:contrastive_loss}.

\paragraph{The InfoMax principle.} Many empirical works are motivated by the InfoMax principle of maximizing $I(f(x); f(y))$ for $(x, y) \sim \ppos$ \citep{tian2019contrastive,bachman2019learning,wu2020importance}. Usually they interpret $\lcontr$ in Eqn.~\eqref{eq:contrastive_loss} as a lower bound of $I(f(x); f(y))$ \citep{oord2018representation,hjelm2018learning,bachman2019learning,tian2019contrastive}. However, this interpretation is known to have issues in practice, \eg, maximizing a tighter bound often leads to worse downstream task performance \citep{tschannen2019mutual}. Therefore, instead of viewing it as a bound, we investigate the exact behavior of directly optimizing $\lcontr$ in the following sections.

==> misc/hypersphere/text/related.tex <==
%auto-ignore
%!TEX root = ../main.tex

% \paragraph{General Contrastive Learning.}

\paragraph{Unsupervised Contrastive Representation Learning} has seen remarkable success in learning representations for image and sequential data \citep{logeswaran2018efficient,wu2018unsupervised,oord2018representation,henaff2019data,tian2019contrastive,hjelm2018learning,bachman2019learning,tian2019contrastive,he2019momentum}. The common motivation behind these work is the InfoMax principle \citep{linsker1988self}, which we here instantiate as maximizing the mutual information (MI) between two views \citep{tian2019contrastive,bachman2019learning,wu2020importance}. However, this interpretation is known to be inconsistent with the actual behavior in practice, \eg, optimizing a tighter bound on MI can lead to worse representations \citep{tschannen2019mutual}. What the contrastive loss exactly achieves remains largely a mystery. Analysis based on the assumption of latent classes provides nice theoretical insights, but unfortunately has a rather large gap with empirical practices \citep{saunshi2019theoretical}. In this paper, we analyze and characterize the behavior of contrastive learning from the perspective of alignment and uniformity properties, and empirically verify our claims with standard representation learning tasks.
%\citet{wu2020importance}

\paragraph{Representation learning on the unit hypersphere. } Outside contrastive learning, many other representation learning approaches also normalize their features to be on the unit hypersphere. In variational autoencoders, the hyperspherical latent space has been shown to perform better than the Euclidean space \citep{xu2018spherical,s-vae18}. Directly matching uniformly sampled points on the unit hypersphere is also known to provide good representations \citep{bojanowski2017unsupervised}, agreeing with our intuition that uniformity is a desirable property. \citet{mettes2019hyperspherical} optimizes prototype representations on the unit hypersphere for classification. Hyperspherical face embeddings also greatly outperform the unnormalized counterparts \citep{parkhi2015deep,liu2017sphereface,wang2017normface,schroff2015facenet}. Its empirical success suggests that the unit hypersphere is indeed a nice feature space. In this work, we formally investigate the interplay between the hypersphere geometry and the popular contrastive representation learning.
%While  \citep{caron2018deep,caron2019leveraging}

\paragraph{Distributing points on the unit hypersphere.}
The problem of uniformly distributing points on the unit (hyper)sphere is a well-studied one. It is often defined as minimizing the total pairwise potential \wrt a certain potential function \citep{borodachov2019discrete,landkof1972foundations}, \eg, the Thomson problem of finding the minimal electrostatic potential energy configuration of electrons \citep{thomson1904xxiv}, and minimization of the Riesz $s$-potential \citep{gotz2001note,hardin2005minimal,liu2018learning}. The uniformity metric we propose is based on the Gaussian potential, which can be used to represent a very general class of kernels and is closely related to the universally optimal point configurations  \citep{borodachov2019discrete,cohn2007universally}. Additionally, the best-packing problem on hyperspheres (often called the Tammes problem) is also well studied \citep{tammes1930origin}.


==> misc/hypersphere/text/structure.tex <==
%auto-ignore
%!TEX root = ../main.tex

\section{Introduction}
\begin{itemize}
    \item Introduce contrastive loss.

    \item Observe that it encourages each feature to be linearly separable with the rest, so they should be extreme points of a convex polytope.

    Plots showing that this is empirically (roughly) true with learned representations via, \eg, CMC.

    \item Observe that symmetry in loss means that they should be uniformly distributed over a hyphersphere\footnote{In reality, each data sample can not be individually mapped, so the resulting embeddings do not exactly form a hypersphere.}.

    Empirically, a number of popular representation learning methods explicitly enforce latent embeddings to live on the unit hypersphere.

    \item Raise two natural questions, which we investigate in this paper: \begin{itemize}
        \item How can we quantify this intuition (uniform over hypersphere)?
        \item What effects does it have on the representation?
    \end{itemize}
\end{itemize}

\section{Why hypersphere?}

\begin{itemize}
    \item Contrastive loss encourages sharp distribution, which can be achieved by simpling scaling the embeddings up.
    \item \textbf{Theorem (Proved)} for arbitrary embedding (directions), contrastive loss can be made arbitrarily close to a lower bound by just scaling them up.
    \item Show empirical correlation between loss and embedding norms.
    \item Therefore, usually embedding vectors are constrained to have bounded / constant norm. And under the bounded norm setting, we can restrict to the case where the norms are maximized, and thus also on the hypersphere.
\end{itemize}

\section{Uniform?}

\begin{itemize}
    \item Quantify, to what extent we can say that contrastive loss is encouraging uniform distribution on the hypersphere.
    \item \textbf{Theorem (Unproved yet, but I feel is close)} The sequence of point configurations on a hypersphere, as the number of points goes to infinity, converges to uniform distribution over the hypersphere.
    \item Show that this empirically true.
\end{itemize}

\section{Why uniform?}

\begin{itemize}
    \item Define representation quality as linear separability.
    \item Argue that connected sets (with smooth boundaries) on the hypersphere are not too far away from a spherical cap, and thus linearly separable.
    \item Empirically verify that this holds for several classes (\eg, on CUBm, where each data point has a number of attributes).
    \item \textbf{Theorem (Unproved yet)} (probably under heavy assumptions) a connect set with nice boundary on a hypersphere is not not too far from a cap.
    \item Show, hopefully, some correlation between a measure of uniformity and classification accuracy over a bunch of trained representations.
\end{itemize}

\section{Improve uniformity}

\begin{itemize}
    \item Investigate auxiliary losses that encourage uniformity, \eg, Reisz potential or Gaussian potential.
    \item Hopefully, show that they help with representation quality, and lie nicely in the correlation plot above..
\end{itemize}


==> misc/hypersphere/text/supplementary__Simon_Wang_s_conflicted_copy_2020-04-22_.tex <==
%auto-ignore
%!TEX root = ../supplementary.tex

\if\fixsubmission1
\section{Errata}

\begin{enumerate}
    \item In the definition of $\lalign$ (occurring at the beginning of Section~4.1.1 and Section~5), the minus sign before expectation is a typo. Instead, the formula should be corrected as \begin{equation}
        \lalign(f; \alpha) = \expectunder[(x, y) \sim \ppos]{\norm{f(x) - f(y)}_2^\alpha},
    \end{equation}\ie, minimizing $\lalign$ encourages positive pairs to have similar features.

    \item In Theorem~1, the result ``the second term is minimized iff $f$ is perfectly uniform'' (line 288 left column) should be more rigorously stated as \begin{equation*}
        \text{``If perfectly uniform encoders exist, they form the exact minimizers of the second term.''}
    \end{equation*}
    We restate the full re-worded version below in Section~\ref{supp:sec:proofs-asymptotics} before its proof.
\end{enumerate}
\fi

\section{Proofs and Additional Theoretical Results}

In this section, we present proofs for propositions and theorems in main paper Sections~4.1.1~and~4.2.

The propositions in Section~4.1.1 illustrate the deep relations between the Gaussian kernel $G_t \colon \sphere^d \times \sphere^d \rightarrow \R$ and the uniform distribution on the unit hypersphere $\sphere^d$. As we will show below in Section~\ref{supp:sec:proof-prop-gauss-unif}, these properties directly follow well-known results on strictly positive definite kernels.

In Section~\ref{supp:sec:proofs-asymptotics}, we present a proof for Theorem~\ref{thm:asym_inf_negatives}. Theorem~\ref{thm:asym_inf_negatives} describes the asymptotic behavior of $\lcontr$ as the number of negative samples goes to infinity, and is strongly related to practical contrastive learning. Empirical practices often use a large number of negatives due to the observation that using more negatives consistently leads to better representation quality \citep{wu2018unsupervised,tian2019contrastive,he2019momentum}. Our proof further reveals connections between $\lcontr$ and $\lunif$ which is defined via the Gaussian kernels.

Finally, we also present a weaker result on the setting where only a single negative is used in $\lcontr$.

\subsection{Proofs for Section~4.1.1} \label{supp:sec:proof-prop-gauss-unif}

To prove Propositions~\ref{supp:prop:continuous-problem}~and~\ref{supp:prop:discrete-problems}, we need to use the \emph{strict positive definiteness} \citep{bochner1992monotone,stewart1976positive} of the Gaussian kernel $G_t$: \begin{equation*}
    G_t(u, v) \trieq e^{-t \norm{u - v}_2^2} = e^{2t \cdot u\T v - 2t}, \quad t > 0.
\end{equation*} From there, we apply a known results on such kernels, which the two propositions directly follow.

\begin{definition}[Strict positive definiteness \citep{bochner1992monotone,stewart1976positive}]
    A symmetric and lower semi-continuous kernel $K$ on $A \times A$ (where $A$ is infinite and compact) is called strictly positive definite if for every finite signed Borel measure $\mu$ supported on $A$ whose energy \begin{equation*}
        I_K[\mu] \trieq \int_u \int_v K(u, v) \diff \mu \diff \mu
    \end{equation*}
    is well defined, we have $I_K[\mu] \geq 0$, where equality holds only if $\mu \equiv 0$ on the $\sigma$-algebra of Borel subsets of $A$.
\end{definition}

\begin{definition}
    Let $\mathcal{M}(\sphere^{d})$ be the set of Borel probability measures on $\sphere^{d}$.
\end{definition}

We are now in the place to apply the following two well-known results, which we present by restating Proposition~4.4.1, Theorem~6.2.1 and Corollary~6.2.2 of \citet{borodachov2019discrete} in weaker forms. We refer readers to \citet{borodachov2019discrete} for their proofs.
\begin{lemma}[Strict positive definiteness of $G_t$] \label{supp:lemma-strict-pd-gaussian}
    For $t > 0$, the Gaussian kernel $G_t \trieq e^{-t \norm{u - v}_2^2} = e^{2t \cdot u\T v - 2t}$ is strictly positive definite  on $\sphere^d \times \sphere^d$.
\end{lemma}

\begin{lemma}[Strictly positive definite kernels on $\sphere^d$] \label{supp:lemma:strict-pd-uniform}
    Consider kernel $K_f \colon \sphere^d \times \sphere^d \rightarrow (-\infty, +\infty]$ of the form, \begin{equation}
        K_f(u, v) \trieq f(\norm{u - v}_2^2).
    \end{equation}
    If $K_f$ is strictly positive definite on $\sphere^d \times \sphere^d $ and $I_{K_f}[\sigma_d]$ is finite, then $\sigma_d$ is the unique measure (on Borel subsets of $\sphere^d$) in the solution of $\min_{\mu \in \mathcal{M}(\sphere^d)} I_{K_f}[\mu]$, and the normalized counting measures associated with any $K_f$-energy minimizing sequence of $N$-point configurations on $\sphere^d$ converges weak$^*$ to $\sigma_d$.

    In particular, this conclusion holds whenever $f$ has the property that $-f'(t)$ is strictly completely monotone on $(0, 4]$ and $I_{K_f}[\sigma_d]$ is finite.
\end{lemma}

\begin{proposition} \label{supp:prop:continuous-problem}
    $\sigma_{d}$ is the unique solution (on Borel subsets of $\sphere^d$) of \begin{equation}
        \min_{\mu \in \mathcal{M}(\sphere^{d})} I_{G_t}[\mu] = \min_{\mu \in \mathcal{M}(\sphere^{d})} \int_u \int_v G_t(u, v) \diff \mu \diff \mu. \label{supp:prop:continuous-problem-solution}
    \end{equation}
\end{proposition}
\begin{proof}[Proof of Proposition~\ref{supp:prop:continuous-problem}]
    This is a direct consequence of Lemmas~\ref{supp:lemma-strict-pd-gaussian}~and~\ref{supp:lemma:strict-pd-uniform}.
\end{proof}

\begin{proposition} \label{supp:prop:discrete-problems}
    For each $N > 0$, the $N$ point minimizer of the average pairwise potential is \begin{equation*}
        \mathbf{u}^*_N = \argmin_{u_1, u_2, \dots, u_N \in \sphere^{d}} \sum_{1 \leq i < j \leq N} G_t(u_i, u_j).
    \end{equation*}
    The normalized counting measures associated with the $\{\mathbf{u}^*_N\}_{N=1}^\infty$ sequence converge weak$^*$ to $\sigma_d$.
\end{proposition}
\begin{proof}[Proof of Proposition~\ref{supp:prop:discrete-problems}]
    This is a direct consequence of Lemmas~\ref{supp:lemma-strict-pd-gaussian}~and~\ref{supp:lemma:strict-pd-uniform}.
\end{proof}

\subsection{Proofs and Additional Results for Section~4.2} \label{supp:sec:proofs-asymptotics}

We will use the following lemmas in our proofs.
\begin{lemma}[Log Linearization] \label{supp:lemma:log_linearization}
    Let $X$ and $Y$ be positive-valued random variables with values with $\supp(Y) \in [\epsilon, \infty)$. Assuming all expectations exist, we have
    \begin{equation*}
        \expect{\log(X) - \log(Y)} \leq \epsilon^{-1} \expect{X - Y}.
    \end{equation*}
\end{lemma}
\begin{proof}
    Due to concavity of $\log(\cdot)$, we have, for $x, y > 0$, \begin{equation*}
        \log(x) \leq \log(y) + (x - y) \log'(y) = \log(y) + \frac{x - y}{y}.
    \end{equation*}
    % Consider the Taylor expansion of function $\log(z)$ about a real number $c > 0$ expressed as, for some $0 < \theta < 1$,  \begin{equation}
    %     \log(z) = \log(c) + (z - c) \log'(\theta c + (1-\theta)z) = \log(c) + \frac{z - c}{\theta c + (1-\theta) z}. \label{supp:thm:log-linearization}
    % \end{equation}
    % Notice that, right-hand-side of Equation~\eqref{supp:thm:log-linearization} is always monotonically increasing in $\theta$.

    Therefore, we have, \begin{equation*}
        \expect{\log(X) - \log(Y)} \leq \expect{\frac{X - Y}{Y}} \leq \epsilon^{-1} \expect{X - Y}.
    \end{equation*}
\end{proof}

We refer readers to \citet{borodachov2019discrete} for proof of the following lemma.
\begin{lemma}[Lemma~1.6.6 of \citet{borodachov2019discrete}] \label{supp:lemma:product_measure_weak_convergence}
    Let $\mu_1, \mu_2, \dots$ be a sequence of finite and positive Borel mea sures supported on a compact set $A \subset \R^p$ that converges weak$^*$ to some finite and positive Borel measure $\mu$ as $n \rightarrow \infty$. Then the sequence of product measures $\{\mu_n \times \mu_n\}_{n=1}^\infty$ converges weak$^*$ to the measure $\mu \times \mu$.
\end{lemma}

\begin{theorem}[Asymptotics of $\lcontr$] \label{thm:asym_inf_negatives}
    As the number of negative samples $M \rightarrow \infty$, the (normalized) contrastive loss converges to \begin{equation}
        \begin{split}
            & \lim_{M \rightarrow \infty} \lcontr(f; \tau, M) - \log M = \\
            & \qquad\qquad\qquad -\frac{1}{\tau} \expectunder[(x, y) \sim \distnpos]{f(x)\T f(y)} + \expectunder[x \sim \distndata]{\log\expectunder[x^- \sim \distndata]{e^{f(x^-)\T f(x) / \tau}}}.
        \end{split}
        \label{eq:contrastive_loss_limit}
    \end{equation}
    We have the following results: \begin{enumerate}
        \item \label{thm:asym_inf_negatives:itm:align} The first term is minimized iff $f$ is perfectly aligned.
        % \item \label{thm:asym_inf_negatives:itm:minima_match} The local minima of the second term are the exact local minima of $\mathcal{L}_\mathsf{unifom}(\wcdot; \tau^{-1})$.
        \item \label{thm:asym_inf_negatives:itm:uniform} If perfectly uniform encoders exist, they form the exact minimizers of the second term.
        %If perfectly uniform encoders exist, they form the exact solutions to minimizing the second term.
    \end{enumerate}
\end{theorem}

\begin{proof}[Proof of Theorem~\ref{thm:asym_inf_negatives}]
We first show Equation~\eqref{eq:contrastive_loss_limit}, and then the two results individually.

\begin{itemize}
    \item \itempara{Proof of Equation~\eqref{eq:contrastive_loss_limit}.}

    Note that for any $x, y \in \R^n$ and $\{x^-_i\}_{i=1}^{M} \iidsim \pdata$, we have \begin{equation}
        \lim_{M \rightarrow \infty} \log\left(\frac{1}{M} e^{f(x)\T f(y) / \tau} + \frac{1}{M} \sum_{i=1}^M e^{f(x^-_i)\T f(x) / \tau} \right) = \log\expectunder[x^- \sim \pdata]{e^{f(x^-)\T f(x) / \tau}} \qquad\text{almost surely}, \label{supp:eq:asymp-inner-convergence-slln}
    \end{equation}
    by the strong law of large numbers (SLLN) and the Continuous Mapping Theorem.

    Then, we can derive
    \begin{equation*}
    \begin{split}
        & \lim_{M \rightarrow \infty} \lcontr(f; \tau, M) - \log M \\
        & \qquad = \expectunder[(x, y) \sim \ppos]{- f(x)\T f(y) / \tau} + \lim_{M \rightarrow \infty} \expectunder[\substack{
            (x, y) \sim \ppos \\
            \{x^-_i\}_{i=1}^{M} \iidsim \pdata
            }]{\log\left(\frac{1}{M} e^{f(x)\T f(y) / \tau}+ \frac{1}{M} \sum_{i=1}^M e^{f(x^-_i)\T f(x) / \tau} \right)} \\
        & \qquad = \expectunder[(x, y) \sim \ppos]{- f(x)\T f(y) / \tau} + \expect{\lim_{M \rightarrow \infty}  \log\left(\frac{1}{M} e^{f(x)\T f(y) / \tau}+ \frac{1}{M} \sum_{i=1}^M e^{f(x^-_i)\T f(x) / \tau} \right)}\\
        & \qquad = -\frac{1}{\tau} \expectunder[(x, y) \sim \ppos]{f(x)\T f(y)} + \expectunder[x \sim \pdata]{\log\expectunder[x^- \sim \pdata]{e^{f(x^-)\T f(x) / \tau}}},
    \end{split}
    \end{equation*}
    where we justify the switching of expectation and limit by the convergence stated in Equation~\eqref{supp:eq:asymp-inner-convergence-slln}, the boundedness of $e^{u\T v/\tau}$ (where $u, v \in \sphere^d, \tau > 0$), and the dominated convergence theorem (DCT).

    \item \itempara{Proof of result~\ref{thm:asym_inf_negatives:itm:align}: The first term is minimized iff $f$ is perfectly aligned.}

    Note that for $u, v \in \sphere^d$, \begin{equation*}
        \norm{u - v}_2^2 = 2 - 2 \cdot u^T v.
    \end{equation*}

    Then the result follows directly the definition of perfect alignment, and the existence of perfectly aligned encoders (\eg, an encoder that maps every input to the same output vector).

    \item \itempara{Proof of result~\ref{thm:asym_inf_negatives:itm:uniform}: If perfectly uniform encoders exist, they form the exact minimizers of the second term.}

    For simplicity, we define the following notation: \begin{definition}
        $\forall \mu \in \mathcal{M}(\sphere^{d})$, $u \in \sphere^d$, \begin{equation}
            U_\mu(u) \trieq \int_{v} e^{u\T v / \tau} \diff \mu(v).
        \end{equation}
    \end{definition}

    Then the second term can be equivalently written as \begin{equation*}
        \expectunder[x \sim \pdata]{\log\expectunder[x^- \sim \pdata]{e^{f(x^-)\T f(x) / \tau}}} = \expectunder[x \sim \pdata]{\log U_{\pdata \circ f^{-1}} (f(x))},
    \end{equation*} where $\pdata \circ f^{-1} \in \mathcal{M}(\sphere^d)$ is the probability measure of features, \ie, the pushforward measure of $\pdata$ via $f$.

    We now consider the following relaxed problem, where the minimization is taken over $\mathcal{M}(\sphere^{d})$, all possible Borel probability measures on the hypersphere: \begin{equation}
        %\min_{\mu \in \mathcal{M}(\sphere^{d})} \int_u  \log \int_v G_{\frac{1}{2\tau}} (u, v) \diff \mu \diff \mu =
        \min_{\mu \in \mathcal{M}(\sphere^{d})} \int_u \log U_\mu(u) \diff \mu.
        \label{supp:eq:thm:inf-neg-unif-relaxed-measure}
    \end{equation}

    Our strategy is to show that the unique minimizer of Equation~\eqref{supp:eq:thm:inf-neg-unif-relaxed-measure} is $\sigma_d$, from which the result~\ref{thm:asym_inf_negatives:itm:uniform} directly follows.

    Let the optimal value be $\log W^*$: \begin{equation*}
        \log W^* = \inf_{\mu \in \mathcal{M}(\sphere^{d})} \int_u  \log U_\mu(u) \diff \mu.
    \end{equation*}

    \begin{itemize}
        \item
        \textbf{First, we show that minimizers in Equation~\eqref{supp:eq:thm:inf-neg-unif-relaxed-measure} exist, \ie, the above infimum is attained for some $\mu\hspace{-10mm} \in \mathcal{M}(\sphere^{d})$.}

        Let $\{\mu_n\}_{n=1}^\infty$ be a sequence in $\mathcal{M}(\sphere^d)$ such that $\lim_{n\rightarrow \infty} \int_u \log U_{\mu_n}(u) \diff {\mu_n} = \log W^*$. From the Helly's Selection Theorem, let $\mu^*$ denote some weak$^*$ cluster point of this sequence. Then $\mu_n$ converges weak$^*$ to $\mu^*$ along a subsequence $n \in \mathcal{N} \subset \N$.

        % \begin{align*}
        %     & \abs{\int_u \log U_{\mu_n}(u) \diff {\mu_n} - \int_u \log U_{\mu^*}(u) \diff \mu^*} \\
        %     & \qquad\leq
        %     \abs{\int_u \log U_{\mu_n}(u) \diff {\mu_n} - \int_u \log U_{\mu^*}(u) \diff \mu_n} +
        %     \abs{\int_u \log U_{\mu^*}(u) \diff {\mu_n} - \int_u \log U_{\mu^*}(u) \diff \mu^*} \\
        %     & \qquad\leq
        %     e^{1/\tau}
        %     \abs{\int_u U_{\mu_n}(u) - U_{\mu^*}(u) \diff \mu_n} +
        %     \abs{\int_u \log U_{\mu^*}(u) \diff {\mu_n} - \int_u \log U_{\mu^*}(u) \diff \mu^*} \\
        %     & \qquad\leq
        %     e^{1/\tau}
        %     \abs{\int_u U_{\mu_n}(u) \diff \mu_n - \int_u U_{\mu^*}(u) \diff \mu^*} +
        %     e^{1/\tau}
        %     \abs{\int_u U_{\mu_n}(u) - U_{\mu^*}(u) \diff \mu_n} +
        %     \abs{\int_u \log U_{\mu^*}(u) \diff {\mu_n} - \int_u \log U_{\mu^*}(u) \diff \mu^*}
        %     % & \qquad\leq
        %     % \abs{\int_u \log U_{\mu_n}(u) \diff {\mu_n} - \int_u \log U_{\mu_n}(u) \diff \mu^*} +
        %     % \int_u \abs{\log U_{\mu_n}(u) - \log U_{\mu^*}(u)} \diff \mu^*
        % \end{align*}

        The error term is bounded as following:
        \begin{multline*}
            \abs{\int_u \log U_{\mu_n}(u) \diff {\mu_n} - \int_u \log U_{\mu^*}(u) \diff \mu^*} \leq \\
            \abs{\int_u \log U_{\mu_n}(u) \diff {\mu_n} - \int_u \log U_{\mu^*}(u) \diff \mu_n} +
            \abs{\int_u \log U_{\mu^*}(u) \diff {\mu_n} - \int_u \log U_{\mu^*}(u) \diff \mu^*}.
        \end{multline*}

        In fact, both terms above converge to $0$ in the limit of $n \rightarrow \infty, n \in \mathcal{N}$: \begin{itemize}
            \item
            By Lemma~\ref{supp:lemma:log_linearization}, we have\begin{align*}
                & \abs{\int_u \log U_{\mu_n}(u) \diff {\mu_n} - \int_u \log U_{\mu^*}(u) \diff \mu_n} \\
                & \qquad\qquad\leq
                e^{1/\tau} \abs{\int_u U_{\mu_n}(u) - U_{\mu^*}(u) \diff \mu_n} \\
                & \qquad\qquad\leq
                e^{1/\tau} \abs{\int_u U_{\mu_n}(u) \diff \mu_n - \int_u U_{\mu^*}(u) \diff \mu^*} +
                e^{1/\tau} \abs{\int_u U_{\mu^*}(u) \diff \mu^* - \int_u U_{\mu^*}(u) \diff \mu_n} \\
                & \qquad\qquad=
                e^{1/\tau} \abs{\int_u \int_v e^{u\T v/\tau} \diff \mu_n \diff \mu_n - \int_u \int_v e^{u\T v/\tau} \diff \mu^* \diff \mu^*} +
                e^{1/\tau} \abs{\int_u U_{\mu^*}(u) \diff \mu^* - \int_u U_{\mu^*}(u) \diff \mu_n},
            \end{align*}
            where both terms converge to $0$ along $\mathcal{N}$ due to the weak$^*$ convergence of $\{\mu_n\}_n$ and $\{\mu_n \times \mu_n\}_n$ to $\mu^*$ and $\mu^* \times \mu^*$ respectively (in view of Lemma~\ref{supp:lemma:product_measure_weak_convergence}).

            \item
            By the weak$^*$ convergence of $\{\mu_n\}$ to $\mu^*$ along $\mathcal{N}$, \begin{equation*}
                \lim_{\shortstack{$n \rightarrow \infty$\\$n \in \mathcal{N}$}} \abs{\int_u \log U_{\mu^*}(u) \diff {\mu_n} - \int_u \log U_{\mu^*}(u) \diff \mu^*} = 0.
            \end{equation*}
        \end{itemize}

        Therefore, the limit is \begin{equation*}
            \log W^* = \lim_{\shortstack{$n \rightarrow \infty$\\$n \in \mathcal{N}$}} \int_u \log U_{\mu_n}(u) \diff {\mu_n} = \int_u \log U_{\mu^*}(u) \diff \mu^*,
        \end{equation*}
        and the infimum is attained at $\mu^*$.
    \end{itemize}

    Let $\mu^*$ be any solution of Equation~\eqref{supp:eq:thm:inf-neg-unif-relaxed-measure}: \begin{equation*}
        \mu^* \in \argmin_{\mu \in \mathcal{M}(\sphere^{d})} \int_u  \log U_\mu(u) \diff \mu.
    \end{equation*}

    As we will prove below, $U_{\mu^*}$ must in fact be constant $\mu^*$-almost surely. Concretely, for any $n = 1, 2, 3, \dots$, we will show that the following set is empty: \begin{equation*}
        T_n = \{u \in \sphere^{d} \colon U_{\mu^*}(u) \leq  W^* - \frac{1}{n}\}.
    \end{equation*}

    Assuming the contrary, we consider an arbitrary probability measure $\lambda \in \mathcal{M}(T_n)$. Consider the $\alpha$-mixing between $\mu^*$ and $\lambda$, denoted as $\mu_\alpha = (1 - \alpha) \mu^* + \alpha \lambda \in \mathcal{M}(\sphere^d)$, $\alpha \in (0, 1)$.

    Substituting $\mu_\alpha$ into Equation~\eqref{supp:eq:thm:inf-neg-unif-relaxed-measure}, we consider individually the two terms of \begin{equation*}
        \int_u \log U_{\mu_\alpha} \diff \mu_\alpha
        =
        \alpha \int_u \log U_{\mu_\alpha}(u) \diff \lambda +
        (1-\alpha) \int_u \log U_{\mu_\alpha}(u) \diff \mu^*.
    \end{equation*}

    \begin{itemize}
        \item We have that
        \begin{align*}
            \int_u \log U_{\mu_\alpha}(u) \diff \lambda
            & = \int_u \log \left ( (1-\alpha) U_{\mu^*}(u) + \alpha U_{\lambda}(u) \right) \diff \lambda \\
            & \leq \int_u \log \left ( (1-\alpha) W^* - \frac{1-\alpha}{n} + \alpha e^{1/\tau} \right) \diff \lambda \\
            & = \log \left ( (1-\alpha) W^* - \frac{1-\alpha}{n} + \alpha e^{1/\tau} \right).
        \end{align*}

        \item
        % \begin{align*}
        %     \int_u \log U_{\mu_\alpha}(u) \diff \mu^*
        %     & = \int_u \log \left ( (1-\alpha) U_{\mu^*}(u) + \alpha U_{\delta_{\hat{v}}}(u) \right) \diff \mu^* \\
        %     & = \int_u \log \left ( (1 - \alpha) U_{\mu^*}(u) + \alpha \int_v e^{u\T v / \tau} \diff \delta_{\hat{v}} \right) \diff \mu^* \\
        %     & \leq \int_u \log \left ( (1 - \alpha) U_{\mu^*}(u) + \alpha  e^{1 / \tau} \right) \diff \mu^* \\
        %     & \leq \log\left((1-\alpha)W^* + \alpha e^{1/\tau}\right) \tag{Jensen's by applying $f(y) = e^y(1-\alpha)+\alpha e^{1/\tau}$}.
        % \end{align*}

        % Consider the Taylor expansion of function $\log(z)$ about a real number $c$ expressed as, for some $0 < \theta \leq 1$,  \begin{equation}
        %     \log(z) = \log(c) + (z - c) \log'(\theta c + (1-\theta)z) = \log(c) + \frac{z - c}{\theta c + (1-\theta) z}. \label{supp:thm:log-linearization}
        % \end{equation}

        % Notice that, Equation~\eqref{supp:thm:log-linearization} is monotonic in $\theta$, and that due to concavity of $\log(z)$, we always have \begin{equation*}
        %     \log(c) + \frac{z - c}{\theta c + (1-\theta) z} \evalat{\theta=0}
        %     \leq
        %     \log(z)
        %     \leq
        %     \log(c) + \frac{z - c}{\theta c + (1-\theta) z} \evalat{\theta=1}.
        % \end{equation*}

        Applying Lemma~\ref{supp:lemma:log_linearization}, we have
        \begin{align*}
            \int_u \log U_{\mu_\alpha}(u) \diff \mu^*
            & = \int_u \log U_{\mu_\alpha}(u) - \log U_{\mu^*}(u) \diff \mu^* + \int_u \log U_{\mu^*}(u) \diff \mu^* \\
            & \leq e^{1/\tau} \int_u U_{\mu_\alpha}(u) - U_{\mu^*}(u) \diff \mu^* + \int_u \log U_{\mu^*}(u) \diff \mu^* \\
            & = \alpha e^{1/\tau} \int_u U_{\lambda}(u)- U_{\mu^*}(u)  \diff \mu^* + \int_u \log U_{\mu^*}(u) \diff \mu^* \\
            & = \alpha e^{1/\tau} \left( \int_u U_{\lambda}(u) \diff \mu^* - \int_u U_{\mu^*}(u) \diff \mu^* \right) + \int_u \log U_{\mu^*}(u) \diff \mu^* \\
            & \leq \alpha e^{1/\tau} \left(W^* - \frac{1}{n} - \int_u U_{\mu^*}(u) \diff \mu^* \right) + \int_u \log U_{\mu^*}(u) \diff \mu^* \\
            & < \int_u \log U_{\mu^*}(u) \diff \mu^* \\
            & = \log W^*,
        \end{align*}
        where the last inequality follows from \begin{equation*}
            W^* \leq \exp  \int_u \log U_{\sigma_d}(u) \diff \sigma_d = \int U_{\sigma_d}(u) \diff \sigma_d \leq \int_u U_{\mu^*}(u) \diff \mu^*
        \end{equation*}
        because $\mu^*$ and $\sigma_d$, respectively, are solutions to Equation~\eqref{supp:eq:thm:inf-neg-unif-relaxed-measure} and Equation~\eqref{supp:prop:continuous-problem-solution}.
    \end{itemize}



    Combining both, we have
    \begin{align*}
        \int_u \log U_{\mu_\alpha} \diff \mu_\alpha
        & =
        \alpha \int_u \log U_{\mu_\alpha}(u) \diff \lambda +
        (1-\alpha) \int_u \log U_{\mu_\alpha}(u) \diff \mu^* \\
        & < \alpha \log \left ( (1-\alpha) W^* - \frac{1-\alpha}{n} + \alpha e^{1/\tau} \right) + (1-\alpha) \log W^* \\
        & < \log W^*,
    \end{align*}
    where the last inequality holds since $\alpha$ is arbitrary.

    However, this contradicts the optimality of $\mu^*$. Therefore, we must have each $T_n = \varnothing$ and \begin{equation*}
        \left\{ u \in \sphere^d \colon \log U_{\mu^*}(u) < \log W^* = \int_u \log U_{\mu^*}(u) \mu^* \right\} = \bigcup_n T_n = \varnothing.
    \end{equation*}

    Recall that, due to the optimality of $\mu^*$, we have \begin{align*}
        \log W^*
        & = \int_u \log U_{\mu^*}(u) \diff \mu^* \\
        & =
        \int_{\{u \colon U_{\mu^*}(u) = W^*\}} \log U_{\mu^*}(u) \diff \mu^* +
        \int_{\{u \colon U_{\mu^*}(u) > W^*\}} \log U_{\mu^*}(u) \diff \mu^* \\
        & \geq
        \log W^* \mu^*\left(\{u \colon U_{\mu^*}(u) = W^*\}\right) +
        \log W^* \mu^*\left(\{u \colon U_{\mu^*}(u) > W^*\}\right) \\
        & = \log W^*,
    \end{align*} where the equality must hold, and thus we must have constant $U_{\mu^*}(\cdot)$ $\mu^*$-almost surely.

    % \begin{align*}
    %     \log U_{\mu_\delta}(u)
    %     & = \log \left ( (1 - \delta) \int_v e^{u\T v / \tau} \diff \mu^* + \delta \int_v e^{u\T v / \tau} \diff \lambda \right) \\
    %     & \leq \log \left ( (1 - \delta) \int_v e^{u\T v / \tau} \diff \mu^* + \delta e^{1 / \tau} \right) \\
    %     & \leq \log \left ( (1 - \delta + \delta e^{2 / \tau} ) \int_v e^{u\T v / \tau} \diff \mu^* \right) \\
    %     & \leq \log U_{\mu^*}(u) + \log  (1 - \delta + \delta e^{2 / \tau} ).
    % \end{align*}

    % \begin{align*}
    %     \log U_{\mu_\delta}(u)
    %     & = \log \left ( (1 - \delta) \int_v e^{u\T v / \tau} \diff \mu^* + \delta \int_v e^{u\T v / \tau} \diff \lambda \right) \\
    %     & \leq \log \left ( (1 - \delta) \int_v e^{u\T v / \tau} \diff \mu^* + \delta e^{1 / \tau} \right) \\
    %     & \leq \log \left ( (1 - \delta + \delta e^{2 / \tau} ) \int_v e^{u\T v / \tau} \diff \mu^* \right) \\
    %     & \leq \log U_{\mu^*}(u) + \log  (1 - \delta + \delta e^{2 / \tau} ).
    % \end{align*}
    % \begin{align*}
    %     \log U_{\mu_\delta}(u)
    %     & = \log \left ( (1 - \delta) \int_v e^{u\T v / \tau} \diff \mu^* + \delta \int_v e^{u\T v / \tau} \diff \lambda \right) \\
    %     & \leq \log \left ( (1 - \delta) \int_v e^{u\T v / \tau} \diff \mu^* + \delta \mu^*(T_n) \int_v e^{u\T v / \tau} \diff \mu^* \right) \\
    %     & \leq \log \left ( (1 - \delta + \delta \mu^*(T_n) ) \int_v e^{u\T v / \tau} \diff \mu^* \right) \\
    %     & \leq \log U_{\mu^*}(u) + \log  (1 - \delta + \delta \mu^*(T_n) ).
    % \end{align*}

    % Therefore, the objective for $\mu_\delta$ is
    % \begin{align}
    %     \int_u \log U_{\mu_\delta}(u) \diff \mu_\delta
    %     & = (1 - \delta) \int_u \log U_{\mu_\delta}(u) \diff \mu^* + \delta \int_u \log U_{\mu_\delta}(u) \diff \lambda \\
    %     & \leq \log  (1 - \delta + \mu^*(T_n) ) + (1 - \delta) \int_u \log U_{\mu^*}(u) \diff \mu^* + \delta \int_u \log U_{\mu^*}(u) \diff \lambda \\
    %     & \leq \log  (1 - \delta + \delta \mu^*(T_n) ) + (1 - \delta) \log W^* + \delta (\log W^* - \frac{1}{n}) \\
    %     & = \log  (1 - \delta + \delta \mu^*(T_n) ) + \log W^* - \delta \frac{1}{n} \\
    %     & <
    % \end{align}

    % \hide{
    % By the first variation, we must have $\forall \nu \in \mathcal{M}(\sphere^{d})$: %
    %  \begin{align}
    %     0
    %     & = \frac{\partial}{\partial \alpha}
    %     \int_u \log U_{(1-\alpha) \mu^* + \alpha \nu}(u) \diff ((1-\alpha) \mu^* + \alpha \nu)
    %     \evalat{\alpha=0} \notag\\
    %     & =
    %     \frac{\partial}{\partial \alpha} (1-\alpha)
    %     \int_u \log U_{(1-\alpha) \mu^* + \alpha \nu}(u) \diff \mu^*
    %     \evalat{\alpha=0}
    %     + \frac{\partial}{\partial \alpha} \alpha
    %     \int_u \log U_{(1-\alpha) \mu^* + \alpha \nu}(u) \diff \nu
    %     \evalat{\alpha=0} \notag\\
    %     & =
    %     - \int_u \log U_{(1-\alpha) \mu^* + \alpha \nu}(u) \diff \mu^*
    %     \evalat{\alpha=0}
    %     +
    %     \frac{\partial}{\partial \alpha}
    %     \int_u \log U_{(1-\alpha) \mu^* + \alpha \nu}(u) \diff \mu^*
    %     \evalat{\alpha=0} \notag\\
    %     & \qquad +
    %     \int_u \log U_{(1-\alpha) \mu^* + \alpha \nu}(u) \diff \nu
    %     \evalat{\alpha=0}
    %     +
    %     0 \cdot \frac{\partial}{\partial \alpha}
    %     \int_u \log U_{(1-\alpha) \mu^* + \alpha \nu}(u) \diff \nu
    %     \evalat{\alpha=0} \notag\\
    %     & =
    %     - \int_u \log U_{\mu^*}(u) \diff \mu^*
    %     +
    %     \int_u \frac{U_{\nu}(u) - U_{\mu^*}(u)}{U_{\mu^* }(u)} \diff \mu^*
    %     +
    %     \int_u \log U_{\mu^*}(u) \diff \nu
    %     +
    %     0 \cdot
    %     \int_u \frac{U_{\nu}(u) - U_{\mu^*}(u)}{U_{\mu^* }(u)} \diff \nu \notag\\
    %     & =
    %     \int_u \frac{U_{\nu}(u)}{U_{\mu^* }(u)} \diff \mu^*
    %     +
    %     \int_u \log U_{\mu^*}(u) \diff (\nu - \mu^*) - 1 \label{supp:thm:asym-inf-neg:eq:alpha-first-variation}.
    % \end{align}

    % Let $\{v_1, v_2, \dots\}$ be a sequence of points on $\sphere^d$ such that \begin{equation*}
    %     \lim_{n \rightarrow \infty} U_{\mu^*}(v_n) = \sup_{v \in \sphere^d} U_{\mu^*}(v),
    % \end{equation*} where the right-hand-side must exist since $U_{\mu^*}$ is bounded above.

    % Consider the sequence of measures $\{\nu_1, \nu_2, \dots\}$ such that $\forall n$, $\nu_n$ is the Dirac measure of $v_n \in \sphere^d$, \ie,  \begin{equation*}
    %     \nu_i \equiv \delta_{v_n}\qquad \in \mathcal{M}(\sphere^d).
    % \end{equation*}

    % Equation~\eqref{supp:thm:asym-inf-neg:eq:alpha-first-variation} gives that $\forall n$, \begin{align*}
    %     1
    %     & = \int_u \frac{U_{\nu_n}(u)}{U_{\mu^* }(u)} \diff \mu^*
    %     +
    %     \int_u \log U_{\mu^*}(u) \diff (\nu_n - \mu^*) \\
    %     & =
    %     \int_u \frac{e^{u\T v_n}}{U_{\mu^* }(u)} \diff \mu^*
    %     +
    %     \log U_{\mu^*}(v_n)
    %     -
    %     \int_u \log U_{\mu^*}(u) \diff \mu^* \\
    %     & \geq
    %     \int_u \frac{e^{u\T v_n}}{\sup_{v \in \sphere^d} U_{\mu^*}(v)} \diff \mu^*
    %     +
    %     \log U_{\mu^*}(v_n)
    %     -
    %     \int_u \log U_{\mu^*}(u) \diff \mu^* \\
    %     & \geq
    %     \frac{U_{\mu^*}(v_n)}{\sup_{v \in \sphere^d} U_{\mu^*}(v)}
    %     +
    %     \log U_{\mu^*}(v_n)
    %     -
    %     \int_u \log U_{\mu^*}(u) \diff \mu^*.
    % \end{align*}

    % Taking the limit of $n \rightarrow \infty$ on both sides, we have \begin{align*}
    %     1 = \lim_{n \rightarrow \infty} 1
    %     & \geq
    %     \lim_{n \rightarrow \infty}
    %     \frac{U_{\mu^*}(v_n)}{\sup_{v \in \sphere^d} U_{\mu^*}(v)}
    %     +
    %     \log U_{\mu^*}(v_n)
    %     -
    %     \int_u \log U_{\mu^*}(u) \diff \mu^* \\
    %     & = 1
    %     +
    %     \log \sup_{v \in \sphere^d} U_{\mu^*}(v)
    %     -
    %     \int_u \log U_{\mu^*}(u) \diff \mu^* \\
    %     & \geq 1,
    % \end{align*}where the last inequality holds because the supremum is greater than the average.

    % Since $1=1$, all equalities must hold. In particular, \begin{equation*}
    %     \log \sup_{v \in \sphere^d} U_{\mu^*}(v) = \int_u \log U_{\mu^*}(u) \diff \mu^*.
    % \end{equation*}
    % That is, for any solution $\mu^*$ of Equation~\eqref{supp:eq:thm:inf-neg-unif-relaxed-measure}, $U_{\mu^*}(u)$ must be constant over $u \in \sphere^d$.
    % }

    Let $S \subset \mathcal{M}(\sphere^d)$ be the set of measures where the above property holds: \begin{equation*}
        S \trieq \left\{\mu \in \mathcal{M}(\sphere^{d}) \colon U_{\mu}(\cdot) \text{ is constant $\mu$-almost surely} \right\}.
    \end{equation*}

    The problem in Equation~\eqref{supp:eq:thm:inf-neg-unif-relaxed-measure} is equivalent to minimizing over $S$: \begin{align*}
        \argmin_{\mu \in \mathcal{M}(\sphere^{d})} \int_u  \log U_\mu(u) \diff \mu
        & = \argmin_{\mu \in S} \int_u  \log U_\mu(u) \diff \mu \\
        & = \argmin_{\mu \in S} \log \int_u U_\mu(u) \diff \mu \\
        & = \argmin_{\mu \in S} \log \int_u \int_v e^{u\T v / \tau} \diff \mu \diff \mu \\
        & = \argmin_{\mu \in S} \left( \frac{1}{\tau} + \log  \int_u\int_v e^{-\frac{1}{2 \tau} \norm{u - v}^2} \diff \mu \diff \mu \right) \\
        & = \argmin_{\mu \in S} \int_u \int_v G_{\frac{1}{2\tau}}(u, v) \diff \mu \diff \mu.
    \end{align*}

    By Proposition~\ref{supp:prop:continuous-problem} and $\tau > 0$, we know that the uniform distribution $\sigma_d$ is the unique solution to \begin{equation}
        \argmin_{\mu \in \mathcal{M}(\sphere^d)} \int_u \int_v G_{\frac{1}{2\tau}}(u, v) \diff \mu \diff \mu. \label{supp:thm:asymp-inf-neg:eq:unif-equiv-gaussian-prob}
    \end{equation}

    Since $\sigma_d \in S$, it must also be the unique solution to Equation~\eqref{supp:eq:thm:inf-neg-unif-relaxed-measure}.

    If perfectly uniform encoders exist, $\sigma_d$ is realizable, and they are the exact encoders that realize it. Hence, in such cases, they are the exact minimizers of \begin{equation*}
        \min_f \expectunder[x \sim \pdata]{\log\expectunder[x^- \sim \pdata]{e^{f(x^-)\T f(x) / \tau}}}.
    \end{equation*}
\end{itemize}
\end{proof}

\paragraph{Relation between Theorem~\ref{thm:asym_inf_negatives}, $\lalign$ and $\lunif$.} The first term of Equation~\eqref{eq:contrastive_loss_limit} is equivalent with $\lalign$ when $\alpha = 2$, up to a constant and a scaling. In the above proof, we showed that the second term favors uniformity, via the feature distribution that minimizes the pairwise Gaussian kernel (see Equation~\eqref{supp:thm:asymp-inf-neg:eq:unif-equiv-gaussian-prob}): \begin{equation}
    \argmin_{\mu \in \mathcal{M}(\sphere^d)} \int_u \int_v G_{\frac{1}{2\tau}}(u, v) \diff \mu \diff \mu, \label{supp:eq:asym-inf-neg-unif-term-measure-relax}
\end{equation} which can be alternatively viewed as the relaxed problem of optimizing for the uniformity loss: \begin{equation}
    \argmin_f \lunif(f; \frac{1}{2\tau}) = \argmin_f \expect[x, y \iidsim \distndata] {G_{\frac{1}{2\tau}}(f(x), f(y))}. \label{supp:eq:asym-inf-neg-unif-term-realizable-nonrelax}
\end{equation} The relaxation comes from the observation that Equation~\eqref{supp:eq:asym-inf-neg-unif-term-measure-relax} minimizes over all feature distributions on $\sphere^d$, while Equation~\eqref{supp:eq:asym-inf-neg-unif-term-realizable-nonrelax} only considers the realizable ones.

\begin{theorem}[Single negative sample] \label{thm:asym_single_negative}
    If perfectly aligned and uniform encoders exist, they form the exact minimizers of the contrastive loss $\lcontr(f; \tau, M=1)$.
\end{theorem}
\begin{proof}[Proof of Theorem~\ref{thm:asym_single_negative}]
    Since $M=1$, we have \begin{align}
        \lcontr(f; \tau, 1)
        & = \expectunder[\substack{
            (x, y) \sim \ppos \\
            x^- \sim \pdata
            }]{-\frac{1}{\tau} f(x)\T f(y) + \log \left( e^{f(x)\T f(y) / \tau}+  e^{f(x^-)\T f(x) / \tau} \right)} \notag \\
        & \geq \expectunder[\substack{
            x \sim \pdata \\
            x^- \sim \pdata
            }]{-\frac{1}{\tau} + \log \left( e^{1 / \tau}+  e^{f(x^-)\T f(x) / \tau} \right)}\label{supp:thm:single-neg:eq:align-relax} \\
        & \geq -\frac{1}{\tau} + \min_{\mu \in \mathcal{M}(\sphere^d)} \int_u \int_v \log \left( e^{1 / \tau}+  e^{u\T v / \tau} \right) \diff \mu(u) \mu(v) \label{supp:thm:single-neg:eq:unif-relax} \\
        & = -\frac{1}{\tau} + \min_{\mu \in \mathcal{M}(\sphere^d)} \int_u \int_v \log \left( e^{1 / \tau}+  e^{(2 - \norm{u - v}_2^2) / (2 \tau)} \right) \diff \mu(u) \mu(v). \notag
    \end{align}
    By the definition of perfect alignment, the equality in Equation~\eqref{supp:thm:single-neg:eq:align-relax} is satisfied iff $f$ is perfectly aligned.

    Consider function $f \colon (0, 4] \rightarrow \R_+$: \begin{equation*}
        f(t) = \log(e^{\frac{1}{\tau}} + e^{\frac{2 - t}{2\tau}}).
    \end{equation*} It has the following properties: \begin{itemize}
        \item $-f'(t) = \frac{1}{2\tau} \frac{ e^{-\frac{t}{2\tau}} }{1 + e^{-\frac{t}{2\tau}}} = \frac{1}{2\tau} (1 - (1 + e^{-\frac{t}{2\tau}})^{-1})$ is strictly completely monotone on $(0, +\infty)$:

        $\forall t \in (0,  +\infty)$, \begin{align*}
            \frac{1}{2\tau} (1 - (1 + e^{-\frac{t}{2\tau}})^{-1}) & > 0 \\
            (-1)^n \frac{\diff^n }{\diff t^n} \frac{1}{2\tau} (1 - (1 + e^{-\frac{t}{2\tau}})^{-1}) & = \frac{n!}{(2\tau)^{n+1}} (1 + e^{-\frac{t}{2\tau}})^{-(n+1)} > 0, \qquad\qquad n = 1, 2, \dots. \\
        \end{align*}
        \item $f$ is bounded on $(0, 4]$.
    \end{itemize}
    Then, by Lemma~\ref{supp:lemma:strict-pd-uniform}, we have that the equality in Equation~\eqref{supp:thm:single-neg:eq:unif-relax} is satisfied iff the feature distribution induced by $f$ (\ie, the pushforward measure $\pdata \circ f^{-1}$) is $\sigma_d$, that is, in other words, $f$ is perfectly uniform.

    Therefore, \begin{equation*}
        \lcontr(f; \tau, 1) \geq -\frac{1}{\tau} + \int_u \int_v \log \left( e^{1 / \tau}+  e^{u\T v / \tau} \right) \diff \sigma_d(u) \sigma_d(v) = \text{constant independent of $f$},
    \end{equation*}where equality is satisfied iff $f$ is perfectly aligned and uniform. This concludes the proof.
\end{proof}

\paragraph{Difference between Conditions of Theorem~\ref{thm:asym_inf_negatives}~and~\ref{thm:asym_single_negative}.}We remark that the statement in Theorem~\ref{thm:asym_single_negative} is weaker than the previous Theorem~\ref{thm:asym_inf_negatives}. Theorem~\ref{thm:asym_single_negative} is conditioned on the existetnce perfectly aligned and uniform encoders. It shows that $\lcontr(f; \tau, M=1)$ only favors alignment under the condition that perfect uniformity is realizable, and vice versa. In Theorem~\ref{thm:asym_inf_negatives}, $\lcontr$ decomposes into two terms, each favoring alignment and uniformity. Therefore, the decomposition in Theorem~\ref{thm:asym_inf_negatives} is exempt from this constraint.

\section{Experiment Details}
For \cifar, \stl and \nyudepth experiments, we use the following settings (unless otherwise stated): \begin{itemize}
    \item Standard data augmentation procedures are used for generating positive pairs, including resizing, cropping, horizontal flipping, color jittering, and random grayscale conversion. This follows prior empirical work in contrastive representation learning \citep{wu2018unsupervised,tian2019contrastive,hjelm2018learning,bachman2019learning}.
    \item Neural network architectures follow the corresponding experiments on these datasets in \citet{tian2019contrastive}. For \nyudepth evaluation, the architecture of the depth prediction CNN is described in Table~\ref{supp:tbl:nyudepth-cnn-depth-predictor-arch}.
    \item We use minibatch stochastic gradient descent (SGD) with $0.9$ momentum and $0.0001$ weight decay.
    \item We use linearly scaled learning rate ($0.06$ per $256$ batch size) \citep{goyal2017accurate}. \begin{itemize}
        \item \cifar and \stl: Optimization is done over $200$ epochs, with learning rate decayed by a factor of $0.2$ at epochs $155$, $170$, and $185$.
        \item \nyudepth: Optimization is done over $400$ epochs, with learning rate decayed by a factor of $0.2$ at epochs $310$, $340$, and $370$.
    \end{itemize}
    \item Encoders are optimized over the training split. For evaluation, we freeze the encoder, and train classifiers / depth predictors on the training set samples, and test on the validation split. \begin{itemize}
        \item \cifar and \stl: We use standard train-val split. Linears classifier are trained with Adam \citep{kingma2014adam} over $100$ epochs, with a learning rate of $0.001$, decayed by a factor of $0.2$ at epochs $60$ and $80$.
        \item \nyudepth: We use the train-val split on the $1449$ labeled images from \citet{Silberman:ECCV12}. Depth predictors are trained with Adam \citep{kingma2014adam} over $100$ epochs, with a learning rate of $0.003$, decayed by a factor of $0.2$ at epochs $60$, $80$, and $90$.
    \end{itemize}
    \item All experiments are performed on 1-4 NVIDIA Titan Xp, Titan X PASCAL, Titan RTX, or 2080 Ti GPUs.
\end{itemize}

\begin{table*}[t!]%
    \input{figuretext/supplementary/tbl_nyudepth_cnn_arch}
\end{table*}


At each SGD iteration, a minibatch of $K$ positive pairs is sampled $\{(x_i, y_i)\}_{i=1}^K$, and the three losses for this minibatch are calculated as following: \begin{itemize}
    \item $\lcontr$: For each $x_i$, the sample contrastive loss is taken with the positive being $y_i$, and the negatives being $\{y_j\}_{j \neq i}$. For each $y_i$, the sample loss is computed similarly. The minibatch loss is calculated by aggregating these $2K$ terms: \begin{equation*}
        \frac{1}{K} \sum_{i = 1}^{K}
        \log \frac{e^{f(x_i)\T f(y_i) / \tau}}{\sum_{j = 1}^{K} e^{f(x_i)\T f(y_j) / \tau}} +
        \frac{1}{K} \sum_{i = 1}^{K} \log \frac{e^{f(x_i)\T f(y_i) / \tau}}{\sum_{j = 1}^{K} e^{f(x_j)\T f(y_i) / \tau}}.
    \end{equation*} This calculation follows empirical practices and is similar to \citet{oord2018representation,henaff2019data}, and \textit{end-to-end} in \citet{he2019momentum}.
    \item $\lalign$: The minibatch alignment loss is straightforwardly computed as \begin{equation*}
        \frac{1}{K} \sum_{i=1}^{K} \norm{f(x_i) - f(y_i)}_2^\alpha.
    \end{equation*}
    \item $\lunif$: The minibatch uniform loss is calculated by considering each pair of $\{x_i\}_i$ and $\{y_i\}_i$: \begin{equation*}
        \log \bigg( \frac{2}{K (K - 1)} \sum_{i \neq j} e^{-t \norm{f(x_i) - f(x_j)}_2^2} \bigg) + \log \bigg( \frac{2}{K (K - 1)} \sum_{i \neq j} e^{-t \norm{f(y_i) - f(y_j)}_2^2} \bigg).
    \end{equation*}
\end{itemize}

Tables~\ref{supp:tbl:stl10-big}~and~\ref{supp:tbl:nyudepth-big} below describe the full specifications of all \if\fixsubmission1  $260$ \else $263$ \fi \stl and $64$ \nyudepth encoders. These experiment results are visualized in main paper Figure~3, showing a clear connection between representation quality and $\lalign$ \& $\lunif$ metrics.


\newpage
\input{figuretext/supplementary/tbl_stl10}
\vspace{2.5cm}

% \newpage
\input{figuretext/supplementary/tbl_nyudepth}

==> misc/hypersphere/text/theory.tex <==
%auto-ignore
%!TEX root = ../main.tex

\subsection{Limiting Behavior of Contrastive Learning} \label{sec:limit}

In this section, we formalize the intuition that contrastive learning optimizes alignment and uniformity, and characterize its asymptotic behavior. We consider optimization problems over all measurable encoder functions from the $\pdata$ measure in $\R^n$ to the Borel space $\sphere^{m-1}$.


We first define the notion of optimal encoders for each of these two metrics.
% To individually analyze the effects of alignment and uniformity, we focus on the scenario when the encoder can independently optimize each of them.
% \begin{assumption}[Realizability of the ``Ideal'' Encoder]
%     The conditional positive pair distributions $\{\distnpos( y \given x) \colon \forall x\}$ have mutually disjoint supports.
% \end{assumption}

\begin{definition}[Perfect Alignment]
    We say an encoder $f$ is \emph{perfectly aligned} if $f(x) = f(y)$ \asurely over $(x, y) \sim \distnpos$.
\end{definition}

\begin{definition}[Perfect Uniformity]
    We say an encoder $f$ is \emph{perfectly uniform} if %
    %  \wrt Gaussian kernel $G_t$ if \begin{equation}
    %     f \in \argmin_f \lunif(f; t).
    % \end{equation}
    the distribution of $f(x)$ for $x \sim \distndata$ is the uniform distribution $\sigma_{m-1}$ on $\sphere^{m-1}$.
\end{definition}

\paragraph{Realizability of perfect uniformity.} We note that it is not always possible to achieve perfect uniformity, \eg, when the data manifold in $\R^n$ is lower dimensional than the feature space $\sphere^{m-1}$. Moreover, in the case that $\distndata$ and $\distnpos$ are formed from sampling augmented samples from a finite dataset, there cannot be an encoder that is \emph{both} perfectly aligned and perfectly uniform, because perfect alignment implies that all augmentations from a single element have the same feature vector. Nonetheless, perfectly uniform encoder functions do exist under the mild conditions that $n \geq m-1$ and $\distndata$ has bounded density. %Furthermore, even when they may not exist, result~\ref{thm:asym_inf_negatives:itm:minima_match} in the following Theorem~\ref{thm:asym_inf_negatives} still connects the contrastive loss $\lcontr$ with the uniformity loss $\lunif$ defined above.

We first analyze the asymptotics with infinite negative samples. Existing empirical work has established that larger number of negative samples consistently leads to better downstream task performances \citep{wu2018unsupervised,tian2019contrastive,he2019momentum}, and often uses very large values (\eg, $M=65536$ in \citet{he2019momentum}). The following theorem nicely confirms that optimizing \wrt the limiting loss indeed requires both alignment and uniformity.

\begin{theorem}[Asymptotics of $\lcontr$] \label{thm:asym_inf_negatives}
    As the number of negative samples $M \rightarrow \infty$, the (normalized) contrastive loss converges to \begin{equation}
        \begin{split}
        & \lim_{M \rightarrow \infty} \lcontr(f; \tau, M) - \log M = \\
        & \qquad -\frac{1}{\tau} \expectunder[(x, y) \sim \distnpos]{f(x)\T f(y)} \\
        & \qquad + \expectunder[x \sim \distndata]{\log\expectunder[x^- \sim \distndata]{e^{f(x^-)\T f(x) / \tau}}}.
        \end{split}
        \label{eq:contrastive_loss_limit}
    \end{equation}
    We have the following results: \begin{enumerate}
        \item The first term is minimized iff $f$ is perfectly aligned.
        % \item \label{thm:asym_inf_negatives:itm:minima_match} The local minima of the second term are the exact local minima of $\mathcal{L}_\mathsf{unifom}(\wcdot; \tau^{-1})$.
\if\fixsubmission1
        \item The second term is minimized iff $f$ is perfectly uniform.
        %If perfectly uniform encoders exist, they form the exact solutions to minimizing the second term.
\else
        \item If perfectly uniform encoders exist, they form the exact minimizers of the second term.
\fi
    \end{enumerate}
\end{theorem}
\begin{proof}
    See supplementary material.
\end{proof}

% The following corollary directly follows from Theorem~\ref{thm:asym_inf_negatives}.
% \begin{corollary}
%     If perfectly aligned and uniform encoders exist, they are the exact minimizers of the limiting (normalized) contrastive loss $\lim_{M \rightarrow \infty} \lcontr(f; \tau, M) - \log M$.
% \end{corollary}

When $\pdata$ is uniform over finite samples $\{x_1, x_2, \dots, x_N\}$ (\eg, a collected dataset), the second term in Eqn.~\eqref{eq:contrastive_loss_limit} can be alternatively viewed as a resubstitution entropy estimator of $f(x)$ \citep{ahmad1976nonparametric}, where $x$ follows the underlying distribution $p_\mathsf{nature}$ that generates $\{x_i\}_{i=1}^N$, via a von~Mises-Fisher (vMF) kernel density estimation (KDE):%
\begin{align*}
    & \expectunder[x \sim \distndata]{\log\expectunder[x^- \sim \pdata]{e^{f(x^-)\T f(x) / \tau}}} \\
    & \qquad = \frac{1}{N}\sum_{i=1}^N \log \left( \frac{1}{N}\sum_{j=1}^N e^{f(x_i)\T f(x_j) / \tau} \right) \\
    % & \qquad = \frac{1}{N}\sum_{i=1}^N \log \left( \frac{Z_\mathsf{vMF}}{N}\sum_{j=1}^N p_\mathsf{vMF}(f(x_i); f(x_j)) \right) \\
    & \qquad = \frac{1}{N}\sum_{i=1}^N \log \hat{p}_\mathsf{vMF\text{-}KDE}(f(x_i)) + \log Z_\mathsf{vMF} \\
    & \qquad \trieq -\hat{H}(f(x)) + \log Z_\mathsf{vMF}, \qquad\qquad\quad x \sim p_\mathsf{nature} \\
    & \qquad \trieq -\hat{I}(x; f(x)) + \log Z_\mathsf{vMF}, \qquad\quad\hspace{14pt}x \sim p_\mathsf{nature},
\end{align*}%
\vspace{-3pt}where \begin{itemize}
    \item $\hat{p}_\mathsf{vMF\text{-}KDE}$ is the KDE based on samples $\{f(x_j)\}_{j=1}^N$ using a vMF kernel with $\kappa = \tau^{-1}$,
    \item $Z_\mathsf{vMF}$ is the normalization constant for vMF distribution with $\kappa = \tau^{-1}$,
    \item $\hat{H}$ denotes the resubstitution entropy estimator,
    \item $\hat{I}$ denotes the mutual information estimator based on $\hat{H}$, since $f$ is a deterministic function.
\end{itemize}

\paragraph{Relation with the InfoMax principle.}  Many empirical works are motivated by the InfoMax principle, \ie maximizing $I(f(x); f(y))$ for $(x, y) \sim \ppos$.  However, the interpretation of $\lcontr$  as a lower bound of $I(f(x); f(y))$ is known to be inconsistent with the actual behavior in practice \citep{tschannen2019mutual}. Our results instead analyze the properties of $\lcontr$ itself. In particular, both Theorem~\ref{thm:asym_inf_negatives} and the above connection with maximizing an entropy estimator provide alternative intepretations and motivations for $\lcontr$, since a perfectly uniform encoder is indeed most entropic and achieves the largest possible $I(f(x); f(y))$.

Finally, even for the case where only a single negative sample is used (\ie, $M=1$), we can still prove a weaker result, which we describe in details in supplementary material.
% the following weaker result.
% \begin{theorem}[Single negative sample]
%     If perfectly aligned and uniform encoders exist, they form the exact minimizers of the contrastive loss $\lcontr(f; \tau, M=1)$.
% \end{theorem}
% \begin{proof}
%     See supplementary material.
% \end{proof}

% We remark that this statement is weaker than the previous Theorem~\ref{thm:asym_inf_negatives}. It only shows that $\lcontr(f; \tau, M=1)$ favors alignment under the condition that perfect uniformity is realizable, and vice versa. The decomposition in Theorem~\ref{thm:asym_inf_negatives}, however, is exempt from this constraint.

==> text/niceness.tex <==
%auto-ignore
%!TEX root = ../main.tex


\subsection{Why are Uniformity and Alignment Nice?}
\todo{intuition, motivate with class-positive-pair examples, maybe theory}

But why are uniformity and alignment nice properties?

\subsubsection{$\ppos$ and Alignment Affect Class Concentration}

First, we observe hat class concentration naturally happens in unsupervised contrastive learning (\eg, in Figure~\ref{fig:toy2d}), \ie, samples of the same class are mapped to nearby feature vectors.

Some may argue that this is the result of the powerful inductive bias of convolutional neural network (CNN) encoder \citep{cohen2016inductive}. We will show below that the choice of $p_\mathsf{pos}$ and the alignment property also empirically play important roles.

Analogous to $\lalign$, we use the following metric to quantify class concentration. For a label distribution $\pcls$, \begin{equation}
    \lclscon(f) \trieq - \expectunder[c \sim \pcls] {\expectunder[x, y \iidsim \distndata(\cdot \given c)] {\norm{f(x) - f(y)}_2^2}}.%, \quad \alpha > 0.
\end{equation}%
\Ie, the expectation is now taken over sample pairs that share the same class label.

To investigate the effect of $\ppos$ and alignment, we consider four different $\ppos$ choices: \begin{itemize}
    \item Light augmentation: \todo{talk about how this violates matching marginal?}%$\ppos(x, y) = \indic{x = y} \pdata(x)$.
    \item Normal augmentation:
    \item Normal augmentation + sampling from same class.
\end{itemize}
and encoders trained in three different ways: \begin{itemize}
    \item Supervised predictive learning. \todo{fix desc}
    \item Unsupervised contrastive learning with various temperature.
    \item Unsupervised $\lalign$ and $\lunif$ learning with various weights.
\end{itemize}

\todo{talk about class concentration, latent class, relation with alignment}

\subsubsection{Sets on the Hypersphere and Linear Separability}



\todo{visualization of uniform, class, linear separability}
